Interpretable Saliency Maps And Self-Supervised Learning For Generalized Zero Shot Medical Image Classification

In many real world medical image classification settings we do not have access to samples of all possible disease classes, while a robust system is expected to give high performance in recognizing novel test data. We propose a generalized zero shot learning (GZSL) method that uses self supervised learning (SSL) for: 1) selecting anchor vectors of different disease classes; and 2) training a feature generator. Our approach does not require class attribute vectors which are available for natural images but not for medical images. SSL ensures that the anchor vectors are representative of each class. SSL is also used to generate synthetic features of unseen classes. Using a simpler architecture, our method matches a state of the art SSL based GZSL method for natural images and outperforms all methods for medical images. Our method is adaptable enough to accommodate class attribute vectors when they are available for natural images.

==> Misc_method_Ver3.tex <==
\section{Method}
\label{sec:method}



% \subsection{Method Overview}
\subsection{ Method Overview}

Figure~\ref{fig:workflow} depicts our overall proposed workflow. Figure~\ref{fig:workflow} (a) shows the feature extractor network. Given a set of histopathology images,$I^{DP}$, with known Gleason grades and the corresponding set of MR images $I^{MRI}$ from the same patients, our objective is to learn a method to leverage histopathology and MR image features for predicting Gleason grades of a test image which may come from seen and unseen classes (grades).



$I^{DP}$ and $I^{MRI}$ are both passed through \textbf{different} feature generators to obtain feature vectors, denoted as $F^{DP}$ and $F^{MRI}$, which have two uses. The first use is to train a cycleGAN which learns to generate $F^{DP}$ from $F^{MRI}$ and vice versa.
%
The second use of the feature vectors $F^{DP}$ and $F^{MRI}$ is to train a regressor to predict the class label as a real value. The regressor also acts as a discriminator providing feedback to the feature generator to generate features optimized for the task of predicting the Gleason grades.


\textbf{Revisit later}

We have a separate feature synthesizer network which takes as input a base feature vector alongwith its class, and the desired class label of the output feature vector. The generator part generates a feature vector while a regressor acts as a discriminator providing feedback on the output and helping to train the generator. Using this feature synthesizer we generate samples of the seen and unseen classes which are used to train a classifier for predicting label of test images. 


\begin{figure}[t]
 \centering
\begin{tabular}{c}
\includegraphics[height=4cm, width=8.5cm]{Figures/Workflow1.png}  \\
(a)\\
\includegraphics[height=4cm, width=8.5cm]{Figures/FeatureGenerator.png}  \\
(b)\\
\end{tabular}
\caption{(a) Workflow diagram of proposed method; (b) Feature generator network.}
\label{fig:workflow}
\end{figure}


% The work by Huang et al. \cite{HuangDualGAN} describes a Generative Dual
% Adversarial Network (GDAN) which can be considered the state of the art in generative methods for GZSL.  They use three components - a Generator, a
% Regressor and a Discriminator. The core component 
% is the Generator network that can generate various
% visual features conditioned on class labels. 
% The Regressor network acts
% as a deep embedding function, which maps each visual
% feature back to the corresponding class’s semantic feature or attribute vector.
% %
% The Generator and the Regressor network together
% form a dual learning framework, so that they can learn
% from each other through a cyclic consistency loss. 
% The Discriminator network that measures
% the similarity of a visual-textual feature pair, and it
% interacts with the other two networks through a dual adversarial loss. 





% Due to the fact that it is very challenging to obtain meaningful attribute vectors for medical images, we propose a novel architecture that leverages domain knowledge.

 

% Figure~\ref{fig:workflow} shows the different steps of our proposed method. The image is input to a GAN module which generates features that act as input to the ordinal regressor which learns to predict the different severity values. We train this part of the network comprising GAN and regressor together in an end to end manner since we wish to learn features that are optimal for ordinal regression, and pre-trained networks do not provide such optimal feature vectors. 

We also have a discrminator network to determine whether it is the right label or not.




\subsection{Problem Definition and Notations}

We consider the scenario with available histopathology and MR images of PCa with known Gleason grades (e.g., $1,2,3$), and aim to train a network that can correctly classify from the test set (consisting of MR images) samples of unseen  Gleason grades (e.g. $4,5$) in addition to seen grades. The above is a case of generalized zero shot learning and is a realistic scenario since: 1) it is challenging to obtain sufficient labeled histopathology images for a wide variety of disease cases; 2) MRI, being non-interventional,  is easily obtained compared to histopathology images; 3) it is beneficial to make decisions based on the combination of histopathology and MRI since histopathology images provide better information due to their high resolution. The seen classes can be any combination from the Gleason scale. % Although in this example we have taken grades $1,2,3$ as available classes, in reality the available grades can be one or more from the Gleason scale.


Let us denote the dataset of `Seen' classes as 
$S = \{i_s,v_{s},y_s\}$
% $S = \{(\textbf{i}, \textbf{v_i}, y)\}$ 
, where $i_s \in \mathcal{I}_{s}$ is the original image in the set of images from the `Seen' class $\mathcal{I}_s$; $v_{s} \in \mathcal{V}^{s}$ is the image feature vector  and $\mathcal{V}^{s}$ is the set of feature vectors from the seen classes; and $y_s\in \mathcal{Y}_{s}$ is the label of $i_s$ and $v_s$, and $\mathcal{Y}_{s}$ is the set of labels for seen classes. %; $\textbf{s}_y \in \mathcal{A}$ is the attribute vector  (semantic embedding) for class $y$.  
%
% Similarly, we  define the `Unseen' set as 
% set as $U = {i_u, v_u, y_u}$, where $i_u \in \mathcal{I}_{u}$ is the original image from the `Unseen' class $I_{u}$; $v_u \in \mathcal{V}_{u}$  and $\mathcal{V}_{u}$ is the set of image features from the unseen classes; $y_u\in \mathcal{Y}_{u}$, $\mathcal{Y}_{u}$ is the set of image labels for unseen classes, $\mathcal{Y}=\mathcal{Y}_{s} \cup \mathcal{Y}_{u}$, and $\mathcal{Y}_{s} \cap \mathcal{Y}_{u}=\emptyset$. 
Similarly, we  define the `Unseen' set as $U = {i_u, v_u, y_u}$, where $i_u \in \mathcal{I}_{u}$ is the original image from the `Unseen' class $I_{u}$; $v_u$ is the image feature from the set $\mathcal{V}_{u}$; $y_u\in \mathcal{Y}_{u}$, $\mathcal{Y}_{u}$ is the set of image labels for unseen classes, $\mathcal{Y}=\mathcal{Y}_{s} \cup \mathcal{Y}_{u}$, and $\mathcal{Y}_{s} \cap \mathcal{Y}_{u}=\emptyset$.




%Below we describe different components of our proposed network.

% \subsection{Feature Generation Network}
\subsection{Feature Extraction Network}

An important component of state of the art GZSL methods is the availability of a class attribute vector that defines the characteristics of the seen and unseen classes. However in medical images it is extremely challenging to obtain a descriptive attribute vector due to time constraints of clinical experts. Moreover it is not trivial to describe any class (seen or unseen) by class attribute vectors since the same class may have different attribute vectors due to differences in medical conditions. An important novelty of our method is performing GZSL without the need for class attribute vectors.


The first step is to extract features from the histopathology and MR images. We choose to work on image features instead of original images because: 1) output images of generative models can be blurry, especially where there are multiple objects (e.g., multiple cells in histopathology images), and the synthetic images often lack the sharpness to learn discriminative features. Previous works \cite{FelixECCV18,huang7} show that visual representations result in higher classification accuracy in  GZSL compared to images;
%
2) generating high resolution histopathology images from low resolution and noisy MRI is an extremely challenging task and finding a transformation between their feature vectors is much more feasible.


 GZSL approaches applied on natural images use a networked pre-trained on ImageNet \cite{ImageNet} to extract discriminative features since ImageNet covers a wide variety of classes. Finding a corresponding pre-trained network for medical images is challenging since large and diverse datasets are not easily available for all medical imaging modalities. %Furthermore, in our use case we have histopathology and MRI of the same patient, and similar public datasets with both imaging modalities is not  available. 
%
% 
% 
% Although we term our network as a feature generator network, it does not have any generative models like GANs or conditional variational auto encoders. 
%
Figure~\ref{fig:workflow} (b) shows the details of the feature extractor network. A given input image is processed through a ResNet-50 architecture \cite{ResNet50} whose softmax layer has been removed. After going through the $5$ convolution blocks ($conv1-conv5$) we extract the output of the $1000-d$ FC layer. The output of the FC layer (denoted as $fc_{1000}$) is input to a regressor network. 


\subsubsection{Regressor Network}


% We aim to predict Gleason grades which is a form of disease severity where the different classes indicate different levels of known disease severity. A severity label of $1$ indicates absence of disease while the label $5$ indicates the most severe condition. Thus higher class values indicate a progressively increasing severity which can be modeled as a ordinal regression problem. 
%
% Suppose the seen classes are $1,2,3$ and the unknown classes are $4,5$. We train a regressor that learns to predict the different class values. %During the feature generation step for unseen classes the feature vectors are perturbed such that the corresponding regressor output is closer to the unknown classes. The feature vectors are then used to train the network to predict seen and unseen classes.

Every image has an associated label (Gleason grade) which is a discrete value.
However we model the classification problem to one of regression.
%
Instead of regressing input features to the exact class value we incorporate a tolerance parameter $\epsilon$ that allows a certain margin within which the outputs are considered valid, i.e., samples from diseased class $3$ are allowed to have values in the range $[3-\epsilon, 3+\epsilon]$, and the resulting error is zero. %Value of $\epsilon$ controls the degree of robustness of the overall GZSL pipeline.
%
The regressor (Figure~\ref{fig:workflow} (b))  takes as input  $fc_{1000}$, passes it through $3$ hidden fully connected layers consisting of $1024,2048,1024$ neurons respectively and is fed to the output layer without any activation function. The loss function is defined as % a Mean square Error function given by:
%
% \begin{equation}
%     \ell_{regress}= \left\| \widehat{Y}-(Y+\epsilon) \right\|^{2}_2
% \end{equation}
%
\begin{equation}
\ell_{regress}=
\begin{cases}
  \left(|\widehat{Y}-Y|-\epsilon\right).^{2}, & \text{if} ~|\widehat{Y}-Y|> \epsilon 
       \\
  0, & \text{if}~ |\widehat{Y}-Y| \leq \epsilon 
\end{cases}
\end{equation}
%
where $Y$ is the class label, $\widehat{Y}$ is the output of regressor, and $\epsilon$ is the robustness parameter. The above formulation ensures that values of a certain class label $Y$ can map to $Y\pm\epsilon$ with zero error. % that introduces a degree of robustness to the regressor network.  
Our strategy for determining $\epsilon$ is described in Section~\ref{met:synth} with appropriate justification. 


Although our problem is one of classification, converting it to a regression setting has potential advantages. 
% Instead of predicting a fixed class label, the regressor learns to predict a range of values associated with a given severity label. This maps mutliple samples of the same class to a range of values. In turn this provides a degree of control over the feature synthesis step where we can specify the label of output sample and the generated feature would be used accordingly. 
 % perturb feature vectors to produce new features that are closer to the unseen classes as described in (Section~\ref{met:gen}). 
Instead of predicting a fixed class label, the regressor learns to predict a range of values associated with a given Gleason grade. This maps mutliple samples of the same class to a range of values. In turn this provides a degree of control in our downstream task of synthesizing features of unseen classes (Section~\ref{met:synth} where we can specify the desired output label of output sample (as a real value). % and the generated feature would be used accordingly.




\subsubsection{Pre-Training Feature Extraction Network}

We use two separate feature extraction networks for MRI and histopathology images.  
The feature generation component and regression module can be combined as one network and trained simultaneously provided the weights of the convolution blocks can be initialized appropriately. The pre-training scheme is achieved as follows:

\begin{enumerate}
    \item We use a ResNet-34 pre-trained with ImageNet and use the PANDA challenge dataset \cite{Panda} for further weight updates. This public dataset is for the purpose of Gleason grading from whole slide images which is similar to our use case. The ResNet-34 with ImageNet weights helps in faster convergence. Training a network from scratch on the PANDA dataset  does lead to convergence and similar performance levels, but prolongs training time.
    \item The ResNet-34 is trained to correctly predict the Gleason grades with a weighted kappa score of $0.9301$, and a corresponding AUC of $0.9461$. We report the weighted kappa since it is the metric used for leaderboard ranking, and our score places us at rank $11$ of the leaderboard. Our primary aim is to obtain a feature extraction network for histopathology images and not to optimize it to obtain the best results in the challenge. 
    % \item We remove the softmax layer and use the output of the FC layer as the feature vector for our images. This network is further finetuned in an adversarial setting using our image dataset as described in Section~\ref{met:finet}.  
\end{enumerate}

Pre-trained weights for MR images are obtained in the following manner:
\begin{enumerate}
   \item We also employ a ResNet-34 architecture (with ImageNet pre-trained weights) and use the PROMISE12 challenge dataset \cite{Promise12} for further fine-tuning in a self supervised manner. 
   \item This public dataset is for prostate segmentation from MRI and does not have any classification labels. Hence we employ a pre-text task of predicting whether a given image slice contains the prostate or not.
   \item This pre-training using self supervision functions as an effective feature extractor and can be used along with the regression network for the final training. %, Once this pre-training stage is complete we use it to train the entire network end to end. 
   
    % \item This network serves as a feature extractor for our MR images and is further finetuned in an adversarial setting as described in Section~\ref{met:finet}.    
\end{enumerate}

For coupling the feature extractor with the regressor we remove the softmax layer and use the loss function of Eq.~\ref{eq:lreg} for the further training.
After full training of the two feature extractors we have the following components: 1) $FE_{MRI}$ - the feature extractor of MR images that takes an  input MR image and outputs a $1000$ dimensional feature vector $F_{MRI}$; 2) $REG_{MRI}$- the regressor component for MRI images that takes input $F_{MRI}$ and outputs a real value indicating Gleason grade of the sample; 3) $FE_{DP}$ - the feature extractor of digital pathology images that outputs a $1000$ dimensional feature vector $F_{DP}$; 4) $REG_{DP}$- the regressor component for digital pathology images that takes input $F_{DP}$ and outputs a real value indicating Gleason grade of the sample.

% shows the feature generator. The pre-trained feature extraction network is our generator which is denoted as $G:\textbf{I} \xrightarrow[]{} \mathcal{V}$ and parameterized as $\theta_G$. It's output is fed to the discriminator $D$ that provides feedback to the generator and is parameterized as $\theta_D$. 

% The training algorithm for estimating $\theta_G$ and $\theta_D$
% follows a minimax game, where $G(.)$ generates synthetic visual representations
% that are supposed to fool the discriminator, which in turn tries to distinguish the
% real from the synthetic visual representations.


















\subsection{Feature Transformation Network}

Our aim is to predict Gleason grades from MR images. Since Gleason grades are assigned based on the examination of histopathology images it is important to have the corresponding histopathology image for accurate prediction using MRI.% Histopathology images are obtained only after tissue resection which is a much later stage of treatment, while MR images can be easily acquired in a non-interventional manner. 
%
We train a feature transformation network that can generate $F_{DP}$ from its corresponding $F_{MRI}$ using cyclic GANs \cite{CyclicGANS}. Cycle GANs also allow for the reverse transformation.  % which prevents  unconstrained generation of featuresthus improving robustness. 

% Cycle GANs transform an image from domain $ A $ to $B$, and the reverse translation from $ B $ to $ A $ should generate the original input image. 
% %
% In forward cycle consistency, an image from domain $A$ is translated to domain $B$  by generator $G_{AB}$ expressed as $a\hat{b}=G_{AB}(a)$. Image $a\hat{b}$ is translated back to domain $A$ by $G_{BA}$ to get $\hat{a}=G_{BA}(a\hat{b})$.  Similarly, the original and reconstructed images from $B$ should also match.  Thus the overall cycle consistency loss is: % calculated as 
% %
% \begin{equation}
%     L_{cycle} (G_{AB},G_{BA}) = E_{a} \left\|a -G_{BA}(G_{AB}(a))\right\|_1 + \left\|b -G_{AB}(G_{BA}(b))\right\|_1 +L_{Seg},  
%     \label{eq:cyc}
% \end{equation}
%
% where $L_{Seg}$ is defined as 
% \begin{equation}
%     L_{Seg} = \overbrace{L_{FeatMap}(a,\hat{a}) + L_{FeatMap}(b,\hat{b})}^{L_{Seg1}} + \overbrace{L_{FeatMap}(a,a\hat{b}) + L_{FeatMap}(b,b\hat{a})}^{L_{Seg2}}
%     \label{eq:segL}
% \end{equation}
% 
%



%
% Discriminator $D_B$ is employed to distinguish between real image $b$
% and generated image $a\hat{b}$ where the adversarial loss in forward cycle, $L_{adv}$, is:
% %written as
% \begin{equation}
%     L_{adv} (G_{AB},D_{B},A,B) = E_{b} \log D_B (b) +  E_{a} \log \left[ \left(1-D_B (G_{AB}(a))\right)\right].
% \end{equation}
% There also exists a corresponding $L_{adv}(G_{BA},D_A,B,A)$ to distinguish between real image $a$ and generated image $b\hat{a}$
% %
% Thus the final objective function is: %optimized is 
% %
% \begin{equation}
%     L= L_{adv}(G_{AB},D_B,A,B) + L_{adv}(G_{BA},D_A,B,A) + L_{cyc}(G_{AB},G_{BA})
% \end{equation}





CycleGANs \cite{CyclicGANS} learn mapping functions $G : X \rightarrow Y$ and $F : Y \rightarrow X$,  between feature vectors $X=F_{MRI}$ and $Y=F_{DP}$. Adversarial discriminator $D_X$ differentiate  between real features $F_{DP}$ and generated features $\widehat{F}_{DP}$, and $D_Y$ distinguishes between $F_{MRI}$ and $\widehat{F}_{MRI}$. %$\widehat{F}_{DP},\widehat{F}_{MRI}$ are generated histopathology and MRI features. %Here $X=I^{Flt}$ and $Y=I^{Ref}$. 
% $G$ registers $I^{Flt}$ to $I^{Ref}$ while $F$ is trained to register $I^{Ref}$ to $I^{Flt}$. We refer the reader to \cite{CyclicGANs} for implementation details.
%
% In addition to the content loss (Eqn~\ref{eq:conLoss}) we have: 1) an adversarial loss; %to match $I^{Trans}$'s distribution to $I^{Flt}$; 
% and 2) a cycle consistency loss to ensure transformations $G,F$ do not contradict each other.
%
%
%
% \paragraph{\textbf{Adversarial Loss}:}
%
%
The adversarial loss %is an important component to ensure that the generated outputs are plausible. In previous applications the adversarial loss was based on the similarity of generated image to training data distribution. Since our generator network has multiple outputs we have additional terms for the adversarial loss. The first term matches the distribution of $I^{Trans}$ to  $I^{Flt}$  %training data image function ensures that $I^{Trans}$ has similar intensity distribution as $I^{Flt}$, %, and similar spatial shape distribution as , 
 is given by:
%
\begin{equation}
\begin{split}
L_{cycGAN}(G,D_Y) = E_{y\in p_{data}(y)} \left[\log D_Y(y)\right] \\
+ E_{x\in p_{data}(x)} \left[\log \left(1-D_Y(G(x))\right)\right], 
\end{split}
\label{eqn:cyGan1}
\end{equation}
%
We retain notations $X,Y$ for conciseness.
%
%
%%
 There also exists $L_{cycGAN}(F,D_X)$, the corresponding adversarial loss for $F$ and $D_X$ and is given by  %,  = E_{x\in p_{data}(x)} \left[\log D_X(x)\right] +  E_{y\in p_{data}(y)} \left[\log \left(1-D_X(F(y))\right)\right]$.
%
%
\begin{equation}
\begin{split}
L_{cycGAN}(F,D_X) = E_{x\in p_{data}(x)} \left[\log D_X(x)\right] \\ 
+ E_{y\in p_{data}(y)} \left[\log \left(1-D_X(F(y))\right)\right].
\end{split}
\label{eqn:cyGan12}
\end{equation}







Cycle consistency loss ensures that for each $x \in X$ the reverse deformation should bring $x$ back to the original feature, i.e. $x \rightarrow G(x) \rightarrow F(G(x))\approx x$. 
Similar constraints also apply for mapping $F$ and $y$. This is achieved using, % the following conditional loss:
%
%\
%
\begin{equation}
%\begin{split}
L_{cyc}(G,F)= E_{x} \left\|F(G(x))-x\right\|_1 + E_{y} \left\|G(F(y))-y\right\|_1,
%\end{split}
\label{eqn:cyGan2}
\end{equation}
%
%w
%

% Instead of the original images, $I^{Ref}$ and $I^{Flt}$, we use their latent vector representations as input to the generator to obtain $I^{Trans}$. %Although there are two different CAEs for the input image pair, we have a single CycleGAN model 




% \subsubsection{Network Architecture}
\paragraph{Network Architecture}:
%
The generator $G$ is a multi-layer perceptron (MLP) with two hidden layers containing $2048$ nodes each having LeakyReLU \cite{FelixECCV34}, and the output
layer, with $2048$ nodes, has a ReLU activation \cite{FelixECCV35}. The generator weights are initialized with a truncated normal with $\mu=0$, $\sigma=0.01$, and biases initialized to $0$. The discriminator $D$ is also
an MLP consisting of two hidden layers containing $2048$ nodes activated
by LeakyReLU, and the output layer has no activation. $D$'s initialization is same as $G$
 




% \subsection{Discriminator Network}

% So far, the Generator and Regressor already combines
% semantic → visual and visual → semantic methods,
% but it still lacks the ability to learn from a flexible metric
% which can better evaluate the similarity of features. In order
% to incorporate metric learning, the third component of our
% model is a Discriminator network D (as shown in the right
% of Figure 3) that takes as input a visual-semantic feature pair
% (v, s) and output a compatibility score indicating the extent
% to which v belongs to the class characterized by s. The
% Discriminator network learns how to evaluate the closeness


% of an image feature to a class, instead of using a predefined
% metric like L1/L2 distance or cosine similarity.
% In order to train the Discrimiantor to distinguish differ-
% ent types of fake data, inspired by Text-to-Image-GAN [26],
% we also train the Discriminator with two kinds of fake in-
% put, i.e. (G(s, z), s) and (v, s − ), where s − is a randomly
% sampled class’s embedding and s 6 = s − . In addition, we
% add a novel third type of fake input generated by the Re-
% gressor, i.e. (v, R(v)). In this way, not only the CVAE but
% also the Regressor can learn from the Discriminator through
% adversarial training.
% Since GANs are notoriously hard to train, there are
% many methods that try to stabilize the training process of
% GAN [12, 22, 4, 13]. In our model, we apply LS-GAN [22]
% as the training method for adversarial loss for its simplicity
% and effectiveness. Thus the adversarial loss for the Discrim-
% inator of our model can be defined as:



% where the first term is the loss for real samples (v, s), the
% second term stands for the scores of features generated by
% the Generator, the third term stands for the scores of class
% embedding generated by the Regressor, and the last term is
% the control loss which trains the Discriminator to discrimi-
% nate pairs of real image features and real negative class em-
% bedding. The negative sample s − is randomly sampled from
% s −
% the set of training classes {s −
% y |y ∈ Y , s y 6 = s}. Here the
% discriminator D tries to push the scores of real samples to
% 1 and push the scores for generated samples to 0, while the
% generator G tries to push the scores of its synthetic samples
% to 1.
% Also, the adv



% \subsection{Full Objective and Training Procedure}

% In adversarial training, the discriminator is training separately
% from the other two networks, while we train the
% CVAE and Regressor using an overall loss defined as:


% where λ 1 , λ 2 and λ 3 are hyper-parameters that assign
% weight on different parts of the overall loss.
% The training procedure of our GDAN model is as fol-
% lows: we first pretrain CVAE using Equation 2, and then
% train the whole model in an adversarial way using Equa-
% tion 5 and Equation 8. The implementation details will be
% provided in the experiment section.



\subsection{Feature Synthesis Network}
\label{met:synth}

%from felixeccv
A major issue of previous GZSL approaches using generative models \cite{Felix1, 8,9} is the unconstrained nature of the generation process that may produce image representations too far from the real distribution  in the training set. This could lead to a inaccurate multi-class classifier, especially for unseen classes. 
%
Our approach to feature synthesis requires specifying a desired real value cooresponding to he synthesized vector that provides a certain degree of control over in feature generation and leads to overall better results than other methods. The synthesis network has a regression (or discriminator) component and a generator component.

% The
% approach we propose to alleviate this problem consists of constraining the syn-
% thetic visual representations to generate back their original semantic features
% - this regularization has been inspired by the cycle consistency loss [10].
 
 



\subsubsection{Regression Component}

Our aim is to generate samples that would correspond to the desired class value of unknown classes. Conventional approaches such as \cite{ManciniEccv20,FelixEccv18} achieve this by a weighted combination of existing feature vectors of the seen classes. This approach has the inherent danger of generating unrealistic images that affects classifier performance.  A naive approach would be to specify a desired unseen class value that would be output by the regressor for synthetic samples. Since the regressor has not seen the class values of unknown classes , even it predicts an unseen class value, the output will be unreliable.  Instead we propose a progressive generator network that starts with a feature vector of known class value and updates a generator network to generate samples with progressively higher value in the severity scale.

Let us assume that the known classes are $1,3$ and the unknown classes are $2,4,5$. Assuming, $\epsilon=0.3$, the regressor weights can accurately recognize features corresponding to $[0.7,1.3]$ and $[2.7,3.3]$. Suppose we wish to generate feature vectors corresponding to class value $2$, the regressor should learn to predict values between $[1.7-2.3]$. To generate features corresponding to class $1.7$ it is recommended to start with a base feature vector corresponding to $1.3$ and use the generator to generate a new feature vector based on feedback from the regressor which also acts a discriminator. Similarly, we generate features of class value $2.3$ starting from base feature of class value $2.7$. To generate features of class values between $[3.7,4.3]$ we start from base feature of class $3.3$ and move to higher values. However this involves generating for a much larger semantic gap.  
It is easier for the regressor to cover the smaller semantic gap between class values $1.3$ and $1.7$ in a progressive manner than generate, say samples of class value $4.3$ from $1.7$. The fact that disease severities have a progressive relationship  enables us to exploit this property for controlled synthetic  feature generation.

In the worst case scenario we have samples of only one class. Using our progressive generative approach we can generate samples of unknown classes from a single known class although it takes much longer to converge than when we have available samples of more than one class value. 



The feature synthesis network generates features  of seen and unseen classes by training a conditional variational auto encoder (CVAE) shown in Figure~\ref{fig:cvae}. % We feed all the training samples (feature vectors $F_{MRI}$) to $R_{MRI}$ to obtain regressed values $r_{MRI}$. The input to the CVAE is a base feature vector ($F_{MRI}^{input}$) from MR images and the desired label $c$ ($r$ of the output feature vector. The output feature vector, $F_{MRI}^{o}$ is input to regressor $R_{MRI}$ which outputs its class value $r_o$. If the output vector actually belongs to the desired output class then a difference of $\pm\epsilon$ with respect to the class label is acceptable. The regressor also acts as a Discriminator that provides feedback to the generator for weight updates. 
%
%
%
 We feed all the training samples (feature vectors $F_{MRI}$) to $R_{MRI}$ to obtain regressed values $r_{MRI}$.
 The input to the feature synthesizer is $F_{MRI}^{input}$ whose output $F_{MRI}^{output}$  is fed to the regression component to determine whether $F_{MRI}^{output}$ corresponds to desired output class value  $r_{MRI}^{output}$. Note that the regressor of the feature synthesis network is different from $R_{MRI}$. 
%  For training we take pairs of features $F_{MRI}^{input},F_{MRI}^{output}$ and their corresponding  $r_{MRI}^{input},r_{MRI}^{output}$. Using the tuple $F_{MRI}^{input},r_{MRI}^{output}$ as input, and  $F_{MRI}^{output}$ as the desired output we train the CVAE for feature synthesis.
 For ease of explanation and brevity we denote $x=F_{MRI}^{input}, z=F_{MRI}^{output}$ and $c=r_{MRI}^{output}$. %We use notations $x,z,c$ for brevity.
 
 

 
 
 
 %--------------------------------------------------
%  ----------------------------------------------------------------------------------------------

The discriminator/regressor, defined by a probabilistic
model $p_R(c|x)$ with parameters $\theta_R$ , is a feedforward neural network that learns to map the input feature vector $x \in \mathcal{R}^{D}$ to its
corresponding class-value $c \in \mathcal{R}^{1}$ . The regressor
is learned using two sources of data:
\begin{enumerate}
    \item Labeled examples $\{x_n,c_{y_n}\}^{N}_{n=1}$ from the seen class,
on which we can define a supervised loss, given by
 %
 \begin{equation}
 \mathcal{L}_{Sup}(\theta_R)=-\mathbb{E}_{ \{x_n,c_{y_n} \} }\left[ p_R(c_{y_n}|x_n) \right]
 \end{equation}
 
 
 \item Synthesized examples $\widehat{x}$ from the generator, for which
we can define an unsupervised loss, given by
\begin{equation}
 \mathcal{L}_{Unsup}(\theta_R)=-\mathbb{E}_{p_{\theta_G} (\widehat{x}|z,c)p(z)p(c)} \left[ p_R(c|\widehat{x}) \right]
 \end{equation}
 
 
 The unsupervised loss is obtained by 
sampling $z$ from prior $p(z)$, and 
class-value $c$ sampled from empirical distribution $p(c)$. This generates an exemplar for distribution $p_{\theta_G}(\widehat{x}|z,c))$, and we calculate the expectation w.r.t. these distributions. %During this
% phase, we can use attributes both from seen as well as
% unseen classes.
%

Keshari et al. \cite{KeshariCvpr20} show that using 
the Online Batch Triplet Loss (OBTL) and centre loss (CL) 
improves the performance of regression component in GZSL setting.
OBTL helps in generating over complete distributions that improve the network's ability to learn unseen class features, while center loss minmizes deviation from the distribution center. We introduce a self supervised loss that alongwith the margin paramter $\epsilon$ contributes towards better features of unseen class. 

% \begin{equation}
    
% \end{equation}




The overall training objective of the regressor is 
the weighted combination of 
supervised and unsupervised losses:% training objectives
%
\begin{equation}
    \min_{\theta_R} \mathcal{L}_R = \mathcal{L}_{Sup} + \lambda_R \cdot \mathcal{L}_{Unsup}
    \label{eq:lreg}
\end{equation}

The above term optimizes regressor parameters $\theta_R$ that ensures regressor predicts correct class-value even with a noisy signal $\widehat{x}$. It is assumed that generator distribution is fixed.

\end{enumerate}




\subsubsection{Generator Component}


The conditional generator $p_G (x|z,c)$ with parameters $\theta_G$  generates synthetic features to train the classifier.
% Hence the training needs to be designed such
% that the generated class conditional distribution nicely ap-
% proximates the true distribution. 
Denoting VAE encoder as $p_E(z|x)$ with parameters $\theta_E$, and the regressor output distribution as $p_R(c|x)$, the VAE loss function is: given by
% (assuming the regressor to be fixed)
%
\begin{equation}
\begin{split}
    \mathcal{L}_{CVAE}(\theta_E,\theta_G)= -\mathbb{E}_{p_E(z|x),p(c|x)}\left[\log p_G(x|z,c)\right] \\
    + KL(p_E(z|x)||p(z))
\end{split}
\label{eq:lcvae}
\end{equation}
%
where the first term on the R.H.S. is the generator’s reconstruction error and the second term, the KL divergence, encourages VAE posterior (the encoder) to be close to the prior. 
%
 The VAE encoder $p_E(z|x)$, VAE conditional
decoder/generator $p_G(x|z, c)$, and the regressor $p_R(c|x)$ are modeled
as Gaussian distributions. The  latent code $(z, c)$ is represented by disentangled representations $p_E(z|x)$ and $p_R(c|x)$ to avoid posterior collapse \cite{Verma11} .


\paragraph{Discriminator-Driven Learning:}
%
Error back-propagation from the discriminator/regressor improves
generator performance by producing exemplars, $\widehat{x}$  coherent with the class-value $c$. This is achieved using multiple loss functions. The
first generates samples whose regressed class value is close to the desired value and is defined as:% assumes the regressor, has optimal parameters and is defined as:
% any reason for it not regressing to the correct
% value is because of the poor generation by the generator:
%
\begin{equation}
 \mathcal{L}_c(\theta_G)=-\mathbb{E}_{p_G(\widehat{x}|z,c)p(z)p(c)}\left[\log p_R(c|\widehat{x}) \right]   
\end{equation}

The second term combines samples drawn prior $p(z)$ and combined with class-value from $p(c)$, to ensure the synthesized features are similar to the training data
%
\begin{equation}
 \mathcal{L}_{Reg}(\theta_G)=-\mathbb{E}_{p(z)p(c)}\left[\log p_G(\widehat{x}|z,c) \right]   
 \label{eq:lreg}
\end{equation}

The third loss term ensures independence (dis-
entanglement) \cite{Verma11} of $z$ from
the class-value $c$. The encoder 
ensures that the sampling distribution and the one obtained
from the generated exemplar follow the same distribution.
% More formally, we add a loss component,
%
\begin{equation}
 \mathcal{L}_{E}(\theta_G)=-\mathbb{E}_{\widehat{x} \sim p_G (\widehat{x}|z,c)} KL\left[\log p_E(z|\widehat{x})||q(z) \right]   
 \label{eq:le}
\end{equation}
%
The distribution $q(z)$ could be the prior $p(z)$ or the posterior
from a labeled sample $p(z|x_n)$. %, in which case the  class-value ute
% component a y n is used. 
Thus the complete learning objective for the generator and encoder is given by,
%
\begin{equation}
    \min_{\theta_G,\theta_E} \mathcal{L}_{VAE} + \lambda_c \cdot \mathcal{L}_c + \lambda_{reg} \cdot \mathcal{L}_{reg} + \lambda_E \cdot \mathcal{L}_E
    \label{eq:lfinal}
\end{equation}

% The overall learning objective for the conditional auto-
% encoder is a weighted combination of all the components
% discussed above, effectively optimizing parameters to en-
% sure good density estimation. Vanilla conditional genera-
% tive models like conditional VAE [21] and [3] crucially lack
% such a mechanism. The weight are hyperparameters, tuned
% for optimal reconstruction.



%  A common choice for generative models is to use  Generative Adversarial
% Nets (GANs) \cite{GANs}. However, as reported in \cite{Huang30}, conditional variational auto encoders (CVAE) can better map noise vectors to image features.
% In our proposed framework the CVAE consists
% of two parts, an encoder $P_E(F^{output}|F^{input},r^{input})$ that maps the base feature vector $F^{input}$ of known class value $r^{input}$, to an output feature vector $F^{output}$. The second component of the CVAE is the decoder/generator $P_G(F^{input}|F^{output}, c)$ that maps the output vector (or the synthesized feature vector) to a class value 
% data point. The training objective of CVAE is to minimize
% the following loss function:
% \begin{equation}
%     CVAE
% \end{equation}
% where DKL(p||q) represents the Kullback-Leibler divergence
% between two distributions p and q, and P(z) is treated
% as a unit Gaussian distribution.


% However, as pointed out in [41, 40, 8, 21], CVAE is hard
% to train due to the posterior collapse problem. In order to
% mitigate this problem, we follow [31] to disentangle z from
% c, so that the encoder only depends on x (i.e. PG(z|x)), as
% illustrated in the top left of Figure 3. Also, as in [21], we
% add an adversarial loss to help learning better CVAE, which
% we will discuss later. The loss of the conditional variational
% autoencoder (CVAE) used in our model is defined as follows:
% LCVAE(E, G) = E
% Pdata(v,s),PE(z|v)[log PG(v|z, s)] (2)
% − DKL(PE(z|v)||P(z)),

% where v is an image’s visual feature and s is the class embedding
% of v.
% Although generative models like VAE [16] and
% GAN [12] have been proved to be effective in generating
% images, the output images of generative models are still
% blurry for images with complex objects, and the synthetic
% images often lack the sharpness to reveal the detailed attributes
% of objects, which are important for zero-shot learning
% [7]. Hence, instead of generating raw images, we train
% CVAE to generate visual feature v, where the ground truth
% visual features are provided by image classification models
% pretrained on ImageNet [28].



\subsection{Training and Implementation}

% The overall network is optimized in three stages. The first stage optimizes the CVAE loss of Eqn.~\ref{eq:lcvae} using the samples from seen class $S$. In the second stage the regressor loss (Eqn.~\ref{eq:lreg}) is optimzed using the feature vectors $F_{MRI}$ and regressd values. This improves the mapping of generated synthetic data to the corresponding class value.






The network is optimized using the Adam optimizer \cite{Adam}. First the CVAE loss of Eqn.~\ref{eq:lcvae} is pre-trained followed by joint training of regressor and encoder-generator pair in optimizing the loss from Eqn.~\ref{eq:lreg} and Eqn.~\ref{eq:lfinal} till convergence.  Hyerparameters were chosen using a train-validation split with $\lambda_R = 0.1, \lambda_c = 0.1, \lambda_{reg} = 0.1$ and $\lambda_E = 0.1$. 

% , which worked well for most of the experiments.
% It is important to note that the same architecture is used
% across all datasets and no extra data/feature engineering is
% used/performed to improve accuracies, thus showcasing the
% efficacy of the training schedule for this task. The encoder
% is realised using a two-hidden layer feedforward network
% while the decoder and the regressor are modeled as feed-
% forward networks consisting of one hidden layer with 512
% hidden units each.





\subsection{ Evaluation Protocol}


% We define the training dataset as $D_{Tr}=S_{Tr}$, where $S_{Tr}\subset S$ is a subset of the `Seen' classes, and the test dataset is $D_{Te}=S_{Te} \cup U$. $S_{Te} \subset S$ is  the test subset of the `Seen' classes. $S_{Te}$ and $S_{Tr}$ share the class labels. %, and ${S}={S}_{Tr} \cup {S}_{Te}$.
%$\mathcal{S}=\mathcal{S}_{Tr} \cup \mathcal{S}_{Te}$
%
% In GZSL we aim to learn a classifier that maps a given image $\textbf{i}$ ( and its generated image feature vector $\textbf{v}$) to a seen or unseen class, i.e., $f:\textbf{i} \xrightarrow[]{} \mathcal{Y}_{s} \cup \mathcal{Y}_{u}$.


In GZSL we perform classification
when the test set has examples from seen and 
unseen classes. An $80-20$ random split of $S$ is done to obtain training and test splits, $S_{Tr},S_{Te}$, of the seen dataset. $S_{Te}$ and $S_{Tr}$ share the class labels. The full test dataset is $D_{Te}=S_{Te} \cup U$. %$S_{Te} \subset S$ is  the test subset of the `Seen' classes. 
%
The seen class $S$ has samples from $3$ Gleason grades and the unseen class $U$ contains samples from the remaining class. We use all possible combinations of labels in $S$ and $U$.
After training is complete we synthesized samples for all classes of
$S + U$ using the generative model. 
Following standard practice  defined in the
literature for GZSL, average class accuracies are calculated for two settings: 1) $\textbf{A}$: training is performed on synthesized samples of $S+U$ classes and test on $U$. 2) $\textbf{B}$: training is performed on synthesized samples of $S+U$ classes and test on $S_{Te}$. We use a softmax classifier to calculate the per class accuracies. % multi-class linear SVM classifier. 
We also report the harmonic mean defined as 
%
\begin{equation}
    H=\frac{2\times Acc_U \times Acc_S}{Acc_U + Acc_S}
\end{equation}
%
where $Acc_S$ and $Acc_U$ denote the accuracy of images
from seen and unseen classes respectively:


% We use the average per-class
% accuracy. This metric reduces the bias of classes having
% higher examples in the test set, and provides a better mea-
% sure of the model performance [34].
% We shall now discuss the experimental setup for the
% two settings we experiment with: ZSL and GZSL. Let the
% datasets be available in two parts, the labeled examples from
% the seen classes, X S and the unlabeled examples from the
% unseen classes, X U .


% Once the model has been trained, in order to predict the
% label for unseen classes, we can first generate new samples
% for each unseen class, and then combine those synthetic
% samples with other samples in the training data, after which
% we can train any new classifier based on this new dataset
% that contains samples for both seen and unseen classes. 


% 3.4 Learning and Testing
% As shown in [1] the training of a classifier using a potentially unlimited num-
% ber of samples from the seen and unseen classes generated with x ~ G(a, z; $\theta_G$
% )
% produces more accurate classification results compared with multi-modal em-
% bedding models [18–21]. Therefore, we train a final softmax classifier P(y|x, $\theta_C$),
% defined in (4), using the generated visual features by minimizing the negative log
% likelihood loss $\ell_{CLS}$( $\theta_C, \theta_G$
% ), as defined in (3), where $\theta_G$
% has been learned from
% one of the feature learning strategies discussed in Sec. 3.3 - the training of the
% classifier produces $\theta_c$
% . The samples used for training the classifier are generated
% based on the task to be solved. For instance, for ZSL, we only use generated
% visual representations from the set of unseen classes; while for GZSL, we use the
% generated samples from seen and unseen classes.
% Finally, the testing is based on the prediction of a class for an input test
% visual representation x, as follows:
% y = arg max
% y2 e Y
% P(y|x, $\theta$.C
% ), (9)
% where e Y = Y for GZSL or e Y = YU for ZSL.



==> Misc_method_verma.tex <==
\section{Method}
\label{sec:method}



% \subsection{Method Overview}
\subsection{ Method Overview}

Figure~\ref{fig:workflow} depicts our overall proposed workflow. Figure~\ref{fig:workflow} (a) shows the feature extractor network. Given a set of histopathology images,$I^{DP}$, with known Gleason grades and the corresponding set of MR images $I^{MRI}$ from the same patients, our objective is to learn a method to leverage histopathology and MR image features for predicting Gleason grades of a test image which may come from seen and unseen classes (grades).



$I^{DP}$ and $I^{MRI}$ are both passed through \textbf{different} feature generators to obtain feature vectors, denoted as $F^{DP}$ and $F^{MRI}$, which have two uses. The first use is to train a cycleGAN which learns to generate $F^{DP}$ from $F^{MRI}$ and vice versa.
%
The second use of the feature vectors $F^{DP}$ and $F^{MRI}$ is to train a regressor to predict the class label as a real value. The regressor also acts as a discriminator providing feedback to the feature generator to generate features optimized for the task of predicting the Gleason grades.


\textbf{Revisit later}

We have a separate feature synthesizer network which takes as input a base feature vector alongwith its class, and the desired class label of the output feature vector. The generator part generates a feature vector while a regressor acts as a discriminator providing feedback on the output and helping to train the generator. Using this feature synthesizer we generate samples of the seen and unseen classes which are used to train a classifier for predicting label of test images. 


\begin{figure}[t]
 \centering
\begin{tabular}{c}
\includegraphics[height=4cm, width=8.5cm]{Figures/Workflow1.png}  \\
(a)\\
\includegraphics[height=4cm, width=8.5cm]{Figures/FeatureGenerator.png}  \\
(b)\\
\end{tabular}
\caption{(a) Workflow diagram of proposed method; (b) Feature generator network.}
\label{fig:workflow}
\end{figure}


% The work by Huang et al. \cite{HuangDualGAN} describes a Generative Dual
% Adversarial Network (GDAN) which can be considered the state of the art in generative methods for GZSL.  They use three components - a Generator, a
% Regressor and a Discriminator. The core component 
% is the Generator network that can generate various
% visual features conditioned on class labels. 
% The Regressor network acts
% as a deep embedding function, which maps each visual
% feature back to the corresponding class’s semantic feature or attribute vector.
% %
% The Generator and the Regressor network together
% form a dual learning framework, so that they can learn
% from each other through a cyclic consistency loss. 
% The Discriminator network that measures
% the similarity of a visual-textual feature pair, and it
% interacts with the other two networks through a dual adversarial loss. 





% Due to the fact that it is very challenging to obtain meaningful attribute vectors for medical images, we propose a novel architecture that leverages domain knowledge.

 

% Figure~\ref{fig:workflow} shows the different steps of our proposed method. The image is input to a GAN module which generates features that act as input to the ordinal regressor which learns to predict the different severity values. We train this part of the network comprising GAN and regressor together in an end to end manner since we wish to learn features that are optimal for ordinal regression, and pre-trained networks do not provide such optimal feature vectors. 

We also have a discrminator network to determine whether it is the right label or not.




\subsection{Problem Definition and Notations}

We consider the scenario with available histopathology and MR images of PCa with known Gleason grades (e.g., $1,2,3$), and aim to train a network that can correctly classify from the test set (consisting of MR images) samples of unseen  Gleason grades (e.g. $4,5$) in addition to seen grades. The above is a case of generalized zero shot learning and is a realistic scenario since: 1) it is challenging to obtain sufficient labeled histopathology images for a wide variety of disease cases; 2) MRI, being non-interventional,  is easily obtained compared to histopathology images; 3) it is beneficial to make decisions based on the combination of histopathology and MRI since histopathology images provide better information due to their high resolution. The seen classes can be any combination from the Gleason scale. % Although in this example we have taken grades $1,2,3$ as available classes, in reality the available grades can be one or more from the Gleason scale.


Let us denote the dataset of `Seen' classes as 
$S = \{i_s,v_{s},y_s\}$
% $S = \{(\textbf{i}, \textbf{v_i}, y)\}$ 
, where $i_s \in \mathcal{I}_{s}$ is the original image in the set of images from the `Seen' class $\mathcal{I}_s$; $v_{s} \in \mathcal{V}^{s}$ is the image feature vector  and $\mathcal{V}^{s}$ is the set of feature vectors from the seen classes; and $y_s\in \mathcal{Y}_{s}$ is the label of $i_s$ and $v_s$, and $\mathcal{Y}_{s}$ is the set of labels for seen classes. %; $\textbf{s}_y \in \mathcal{A}$ is the attribute vector  (semantic embedding) for class $y$.  
%
% Similarly, we  define the `Unseen' set as 
% set as $U = {i_u, v_u, y_u}$, where $i_u \in \mathcal{I}_{u}$ is the original image from the `Unseen' class $I_{u}$; $v_u \in \mathcal{V}_{u}$  and $\mathcal{V}_{u}$ is the set of image features from the unseen classes; $y_u\in \mathcal{Y}_{u}$, $\mathcal{Y}_{u}$ is the set of image labels for unseen classes, $\mathcal{Y}=\mathcal{Y}_{s} \cup \mathcal{Y}_{u}$, and $\mathcal{Y}_{s} \cap \mathcal{Y}_{u}=\emptyset$. 
Similarly, we  define the `Unseen' set as $U = {i_u, v_u, y_u}$, where $i_u \in \mathcal{I}_{u}$ is the original image from the `Unseen' class $I_{u}$; $v_u$ is the image feature from the set $\mathcal{V}_{u}$; $y_u\in \mathcal{Y}_{u}$, $\mathcal{Y}_{u}$ is the set of image labels for unseen classes, $\mathcal{Y}=\mathcal{Y}_{s} \cup \mathcal{Y}_{u}$, and $\mathcal{Y}_{s} \cap \mathcal{Y}_{u}=\emptyset$.


We define the training dataset as $D_{Tr}=S_{Tr}$, where $S_{Tr}\subset S$ is a subset of the `Seen' classes, and the test dataset is $D_{Te}=S_{Te} \cup U$. $S_{Te} \subset S$ is  the test subset of the `Seen' classes, and ${S}={S}_{Tr} \cup {S}_{Te}$.
%$\mathcal{S}=\mathcal{S}_{Tr} \cup \mathcal{S}_{Te}$
%
In GZSL we aim to learn a classifier that maps a given image $\textbf{i}$ ( and its generated image feature vector $\textbf{v}$) to a seen or unseen class, i.e., $f:\textbf{i} \xrightarrow[]{} \mathcal{Y}_{s} \cup \mathcal{Y}_{u}$.

%Below we describe different components of our proposed network.

% \subsection{Feature Generation Network}
\subsection{Feature Extraction Network}

An important component of state of the art GZSL methods is the availability of a class attribute vector that defines the characteristics of the seen and unseen classes. However in medical images it is extremely challenging to obtain a descriptive attribute vector due to time constraints of clinical experts. Moreover it is not trivial to describe any class (seen or unseen) by class attribute vectors since the same class may have different attribute vectors due to differences in medical conditions. An important novelty of our method is performing GZSL without the need for class attribute vectors.


The first step is to extract features from the histopathology and MR images. We choose to work on image features instead of original images because: 1) output images of generative models can be blurry, especially where there are multiple objects (e.g., multiple cells in histopathology images), and the synthetic images often lack the sharpness to learn discriminative features. Previous works \cite{FelixECCV18,huang7} show that visual representations result in higher classification accuracy in  GZSL compared to images;
%
2) generating high resolution histopathology images from low resolution and noisy MRI is an extremely challenging task and finding a transformation between their feature vectors is much more feasible.


 GZSL approaches applied on natural images use a networked pre-trained on ImageNet \cite{ImageNet} to extract discriminative features since ImageNet covers a wide variety of classes. Finding a corresponding pre-trained network for medical images is challenging since large and diverse datasets are not easily available for all medical imaging modalities. %Furthermore, in our use case we have histopathology and MRI of the same patient, and similar public datasets with both imaging modalities is not  available. 
%
% 
% 
% Although we term our network as a feature generator network, it does not have any generative models like GANs or conditional variational auto encoders. 
%
Figure~\ref{fig:workflow} (b) shows the details of the feature extractor network. A given input image is processed through a ResNet-50 architecture \cite{ResNet50} whose softmax layer has been removed. After going through the $5$ convolution blocks ($conv1-conv5$) we extract the output of the $1000-d$ FC layer. The output of the FC layer (denoted as $fc_{1000}$) is input to a regressor network. 


\subsubsection{Regressor Network}


% We aim to predict Gleason grades which is a form of disease severity where the different classes indicate different levels of known disease severity. A severity label of $1$ indicates absence of disease while the label $5$ indicates the most severe condition. Thus higher class values indicate a progressively increasing severity which can be modeled as a ordinal regression problem. 
%
% Suppose the seen classes are $1,2,3$ and the unknown classes are $4,5$. We train a regressor that learns to predict the different class values. %During the feature generation step for unseen classes the feature vectors are perturbed such that the corresponding regressor output is closer to the unknown classes. The feature vectors are then used to train the network to predict seen and unseen classes.

Every image has an associated label (Gleason grade) which is a discrete value.
However we model the classification problem to one of regression.
%
Instead of regressing input features to the exact class value we incorporate a tolerance parameter $\epsilon$ that allows a certain margin within which the outputs are considered valid, i.e., samples from diseased class $3$ are allowed to have values in the range $[3-\epsilon, 3+\epsilon]$. Value of $\epsilon$ controls the degree of robustness of the overall GZSL pipeline.
%
The regressor (Figure~\ref{fig:workflow} (b))  takes as input  $fc_{1000}$, passes it through $3$ hidden fully connected layers consisting of $1024,2048,1024$ neurons respectively and is fed to the output layer without any activation function. The loss function is a Mean square Error function given by:
%
\begin{equation}
    \ell_{regress}= \left\| \widehat{Y}-(Y+\epsilon) \right\|^{2}_2
\end{equation}
%
where $Y$ is the class label, $\widehat{Y}$ is the output of regressor, and $\epsilon$ is the robustness parameter.% that introduces a degree of robustness to the regressor network.  

Although our problem is one of classification, converting it to a regression setting has potential advantages. 
% Instead of predicting a fixed class label, the regressor learns to predict a range of values associated with a given severity label. This maps mutliple samples of the same class to a range of values. In turn this provides a degree of control over the feature synthesis step where we can specify the label of output sample and the generated feature would be used accordingly. 
 % perturb feature vectors to produce new features that are closer to the unseen classes as described in (Section~\ref{met:gen}). 
Instead of predicting a fixed class label, the regressor learns to predict a range of values associated with a given Gleason grade. This maps mutliple samples of the same class to a range of values. In turn this provides a degree of control in our downstream task of synthesizing features of unseen classes (Section~\ref{met:synth} where we can specify the desired output label of output sample (as a real value). % and the generated feature would be used accordingly.




\subsubsection{Pre-Training Feature Extraction Network}

We use two separate feature extraction networks for MRI and histopathology images.  
The feature generation component and regression module can be combined as one network and trained simultaneously provided the weights of the convolution blocks can be initialized appropriately. The pre-training scheme is achieved as follows:

\begin{enumerate}
    \item We use a ResNet-34 pre-trained with ImageNet and use the PANDA challenge dataset \cite{Panda} for further weight updates. This public dataset is for the purpose of Gleason grading from whole slide images which is similar to our use case. The ResNet-34 with ImageNet weights helps in faster convergence. Training a network from scratch on the PANDA dataset  does lead to convergence and similar performance levels, but prolongs training time.
    \item The ResNet-34 is trained to correctly predict the Gleason grades with a weighted kappa score of $0.9301$, and a corresponding AUC of $0.9461$. We report the weighted kappa since it is the metric used for leaderboard ranking, and our score places us at rank $11$ of the leaderboard. Our primary aim is to obtain a feature extraction network for histopathology images and not to optimize it to obtain the best results in the challenge. 
    % \item We remove the softmax layer and use the output of the FC layer as the feature vector for our images. This network is further finetuned in an adversarial setting using our image dataset as described in Section~\ref{met:finet}.  
\end{enumerate}

Pre-trained weights for MR images are obtained in the following manner:
\begin{enumerate}
   \item We also employ a ResNet-34 architecture (with ImageNet pre-trained weights) and use the PROMISE12 challenge dataset \cite{Promise12} for further fine-tuning in a self supervised manner. 
   \item This public dataset is for prostate segmentation from MRI and does not have any classification labels. Hence we employ a pre-text task of predicting whether a given image slice contains the prostate or not.
   \item This pre-training using self supervision functions as an effective feature extractor and can be used along with the regression network for the final training. %, Once this pre-training stage is complete we use it to train the entire network end to end. 
   
    % \item This network serves as a feature extractor for our MR images and is further finetuned in an adversarial setting as described in Section~\ref{met:finet}.    
\end{enumerate}

For coupling the feature extractor with the regressor we remove the softmax layer and use the loss function of Eq.~\ref{eq:lreg} for the further training.
After full training of the two feature extractors we have the following components: 1) $FE_{MRI}$ - the feature extractor of MR images that takes an  input MR image and outputs a $1000$ dimensional feature vector $F_{MRI}$; 2) $REG_{MRI}$- the regressor component for MRI images that takes input $F_{MRI}$ and outputs a real value indicating Gleason grade of the sample; 3) $FE_{DP}$ - the feature extractor of digital pathology images that outputs a $1000$ dimensional feature vector $F_{DP}$; 4) $REG_{DP}$- the regressor component for digital pathology images that takes input $F_{DP}$ and outputs a real value indicating Gleason grade of the sample.

% shows the feature generator. The pre-trained feature extraction network is our generator which is denoted as $G:\textbf{I} \xrightarrow[]{} \mathcal{V}$ and parameterized as $\theta_G$. It's output is fed to the discriminator $D$ that provides feedback to the generator and is parameterized as $\theta_D$. 

% The training algorithm for estimating $\theta_G$ and $\theta_D$
% follows a minimax game, where $G(.)$ generates synthetic visual representations
% that are supposed to fool the discriminator, which in turn tries to distinguish the
% real from the synthetic visual representations.


















\subsection{Feature Transformation Network}

Our aim is to predict Gleason grades from MR images. Since Gleason grades are assigned based on the examination of histopathology images it is important to have the corresponding histopathology image for accurate prediction using MRI.% Histopathology images are obtained only after tissue resection which is a much later stage of treatment, while MR images can be easily acquired in a non-interventional manner. 
%
We train a feature transformation network that can generate $F_{DP}$ from its corresponding $F_{MRI}$ using cyclic GANs \cite{CyclicGANS}. Cycle GANs also allow for the reverse transformation.  % which prevents  unconstrained generation of featuresthus improving robustness. 

% Cycle GANs transform an image from domain $ A $ to $B$, and the reverse translation from $ B $ to $ A $ should generate the original input image. 
% %
% In forward cycle consistency, an image from domain $A$ is translated to domain $B$  by generator $G_{AB}$ expressed as $a\hat{b}=G_{AB}(a)$. Image $a\hat{b}$ is translated back to domain $A$ by $G_{BA}$ to get $\hat{a}=G_{BA}(a\hat{b})$.  Similarly, the original and reconstructed images from $B$ should also match.  Thus the overall cycle consistency loss is: % calculated as 
% %
% \begin{equation}
%     L_{cycle} (G_{AB},G_{BA}) = E_{a} \left\|a -G_{BA}(G_{AB}(a))\right\|_1 + \left\|b -G_{AB}(G_{BA}(b))\right\|_1 +L_{Seg},  
%     \label{eq:cyc}
% \end{equation}
%
% where $L_{Seg}$ is defined as 
% \begin{equation}
%     L_{Seg} = \overbrace{L_{FeatMap}(a,\hat{a}) + L_{FeatMap}(b,\hat{b})}^{L_{Seg1}} + \overbrace{L_{FeatMap}(a,a\hat{b}) + L_{FeatMap}(b,b\hat{a})}^{L_{Seg2}}
%     \label{eq:segL}
% \end{equation}
% 
%



%
% Discriminator $D_B$ is employed to distinguish between real image $b$
% and generated image $a\hat{b}$ where the adversarial loss in forward cycle, $L_{adv}$, is:
% %written as
% \begin{equation}
%     L_{adv} (G_{AB},D_{B},A,B) = E_{b} \log D_B (b) +  E_{a} \log \left[ \left(1-D_B (G_{AB}(a))\right)\right].
% \end{equation}
% There also exists a corresponding $L_{adv}(G_{BA},D_A,B,A)$ to distinguish between real image $a$ and generated image $b\hat{a}$
% %
% Thus the final objective function is: %optimized is 
% %
% \begin{equation}
%     L= L_{adv}(G_{AB},D_B,A,B) + L_{adv}(G_{BA},D_A,B,A) + L_{cyc}(G_{AB},G_{BA})
% \end{equation}





CycleGANs \cite{CyclicGANS} learn mapping functions $G : X \rightarrow Y$ and $F : Y \rightarrow X$,  between feature vectors $X=F_{MRI}$ and $Y=F_{DP}$. Adversarial discriminator $D_X$ differentiate  between real features $F_{DP}$ and generated features $\widehat{F}_{DP}$, and $D_Y$ distinguishes between $F_{MRI}$ and $\widehat{F}_{MRI}$. %$\widehat{F}_{DP},\widehat{F}_{MRI}$ are generated histopathology and MRI features. %Here $X=I^{Flt}$ and $Y=I^{Ref}$. 
% $G$ registers $I^{Flt}$ to $I^{Ref}$ while $F$ is trained to register $I^{Ref}$ to $I^{Flt}$. We refer the reader to \cite{CyclicGANs} for implementation details.
%
% In addition to the content loss (Eqn~\ref{eq:conLoss}) we have: 1) an adversarial loss; %to match $I^{Trans}$'s distribution to $I^{Flt}$; 
% and 2) a cycle consistency loss to ensure transformations $G,F$ do not contradict each other.
%
%
%
% \paragraph{\textbf{Adversarial Loss}:}
%
%
The adversarial loss %is an important component to ensure that the generated outputs are plausible. In previous applications the adversarial loss was based on the similarity of generated image to training data distribution. Since our generator network has multiple outputs we have additional terms for the adversarial loss. The first term matches the distribution of $I^{Trans}$ to  $I^{Flt}$  %training data image function ensures that $I^{Trans}$ has similar intensity distribution as $I^{Flt}$, %, and similar spatial shape distribution as , 
 is given by:
%
\begin{equation}
\begin{split}
L_{cycGAN}(G,D_Y) = E_{y\in p_{data}(y)} \left[\log D_Y(y)\right] \\
+ E_{x\in p_{data}(x)} \left[\log \left(1-D_Y(G(x))\right)\right], 
\end{split}
\label{eqn:cyGan1}
\end{equation}
%
We retain notations $X,Y$ for conciseness.
%
%
%%
 There also exists $L_{cycGAN}(F,D_X)$, the corresponding adversarial loss for $F$ and $D_X$ and is given by  %,  = E_{x\in p_{data}(x)} \left[\log D_X(x)\right] +  E_{y\in p_{data}(y)} \left[\log \left(1-D_X(F(y))\right)\right]$.
%
%
\begin{equation}
\begin{split}
L_{cycGAN}(F,D_X) = E_{x\in p_{data}(x)} \left[\log D_X(x)\right] \\ 
+ E_{y\in p_{data}(y)} \left[\log \left(1-D_X(F(y))\right)\right].
\end{split}
\label{eqn:cyGan12}
\end{equation}







Cycle consistency loss ensures that for each $x \in X$ the reverse deformation should bring $x$ back to the original feature, i.e. $x \rightarrow G(x) \rightarrow F(G(x))\approx x$. 
Similar constraints also apply for mapping $F$ and $y$. This is achieved using, % the following conditional loss:
%
%\
%
\begin{equation}
%\begin{split}
L_{cyc}(G,F)= E_{x} \left\|F(G(x))-x\right\|_1 + E_{y} \left\|G(F(y))-y\right\|_1,
%\end{split}
\label{eqn:cyGan2}
\end{equation}
%
%w
%

% Instead of the original images, $I^{Ref}$ and $I^{Flt}$, we use their latent vector representations as input to the generator to obtain $I^{Trans}$. %Although there are two different CAEs for the input image pair, we have a single CycleGAN model 




% \subsubsection{Network Architecture}
\paragraph{Network Architecture}:
%
The generator $G$ is a multi-layer perceptron (MLP) with two hidden layers containing $2048$ nodes each having LeakyReLU \cite{FelixECCV34}, and the output
layer, with $2048$ nodes, has a ReLU activation \cite{FelixECCV35}. The generator weights are initialized with a truncated normal with $\mu=0$, $\sigma=0.01$, and biases initialized to $0$. The discriminator $D$ is also
an MLP consisting of two hidden layers containing $2048$ nodes activated
by LeakyReLU, and the output layer has no activation. $D$'s initialization is same as $G$
 




% \subsection{Discriminator Network}

% So far, the Generator and Regressor already combines
% semantic → visual and visual → semantic methods,
% but it still lacks the ability to learn from a flexible metric
% which can better evaluate the similarity of features. In order
% to incorporate metric learning, the third component of our
% model is a Discriminator network D (as shown in the right
% of Figure 3) that takes as input a visual-semantic feature pair
% (v, s) and output a compatibility score indicating the extent
% to which v belongs to the class characterized by s. The
% Discriminator network learns how to evaluate the closeness


% of an image feature to a class, instead of using a predefined
% metric like L1/L2 distance or cosine similarity.
% In order to train the Discrimiantor to distinguish differ-
% ent types of fake data, inspired by Text-to-Image-GAN [26],
% we also train the Discriminator with two kinds of fake in-
% put, i.e. (G(s, z), s) and (v, s − ), where s − is a randomly
% sampled class’s embedding and s 6 = s − . In addition, we
% add a novel third type of fake input generated by the Re-
% gressor, i.e. (v, R(v)). In this way, not only the CVAE but
% also the Regressor can learn from the Discriminator through
% adversarial training.
% Since GANs are notoriously hard to train, there are
% many methods that try to stabilize the training process of
% GAN [12, 22, 4, 13]. In our model, we apply LS-GAN [22]
% as the training method for adversarial loss for its simplicity
% and effectiveness. Thus the adversarial loss for the Discrim-
% inator of our model can be defined as:



% where the first term is the loss for real samples (v, s), the
% second term stands for the scores of features generated by
% the Generator, the third term stands for the scores of class
% embedding generated by the Regressor, and the last term is
% the control loss which trains the Discriminator to discrimi-
% nate pairs of real image features and real negative class em-
% bedding. The negative sample s − is randomly sampled from
% s −
% the set of training classes {s −
% y |y ∈ Y , s y 6 = s}. Here the
% discriminator D tries to push the scores of real samples to
% 1 and push the scores for generated samples to 0, while the
% generator G tries to push the scores of its synthetic samples
% to 1.
% Also, the adv



% \subsection{Full Objective and Training Procedure}

% In adversarial training, the discriminator is training separately
% from the other two networks, while we train the
% CVAE and Regressor using an overall loss defined as:


% where λ 1 , λ 2 and λ 3 are hyper-parameters that assign
% weight on different parts of the overall loss.
% The training procedure of our GDAN model is as fol-
% lows: we first pretrain CVAE using Equation 2, and then
% train the whole model in an adversarial way using Equa-
% tion 5 and Equation 8. The implementation details will be
% provided in the experiment section.



\subsection{Feature Synthesis Network}
\label{met:synth}

%from felixeccv
A major issue of previous GZSL approaches using generative models \cite{Felix1, 8,9} is the unconstrained nature of the generation process that may produce image representations too far from the real distribution  in the training set. This could lead to a inaccurate multi-class classifier, especially for unseen classes. 
%
Our approach to feature synthesis requires specifying a desired real value of the synthesized vector that provides a certain degree of control over in feature generation and leads to overall better results than other methods. The synthesis network has a regression (or discriminator) component and a generator component.

% The
% approach we propose to alleviate this problem consists of constraining the syn-
% thetic visual representations to generate back their original semantic features
% - this regularization has been inspired by the cycle consistency loss [10].
 
 



\subsubsection{Regression Component}

The feature synthesis network generates features  of seen and unseen classes by training a conditional variational auto encoder (CVAE) shown in Figure~\ref{fig:cvae}. The input to the CVAE is a base feature vector ($F_{MRI}^{i}$) from MR images and the desired label $c$ of the output feature vector. The output feature vector, $F_{MRI}^{o}$ is input to regressor $R_{MRI}$ which outputs its class value $r_o$. If the output vector actually belongs to the desired output class then a difference of $\pm\epsilon$ with respect to the class label is acceptable. The regressor also acts as a Discriminator that provides feedback to the generator for weight updates. 

Note that the regressor of the feature synthesis network is different from 

For training the CVAE we feed all the training samples (feature vectors $F_{MRI}$) to $R_{MRI}$ to obtain a regressed value $r_{MRI}$ for every training sample. For training we take pairs of features $F_{MRI}^{input},F_{MRI}^{output}$ and their corresponding  $r_{MRI}^{input},r_{MRI}^{output}$. Using the triplet of $F_{MRI}^{input},r_{MRI}^{input},r_{MRI}^{output}$ as input, and  $F_{MRI}^{output}$ as the desired output we train the CVAE for feature synthesis.
 For ease of explanation and brevity we denote $x=F_{MRI}^{input}, z=F_{MRI}^{output}$ and $c=r_{MRI}^{output}$. %We use notations $x,z,c$ for brevity.
 
 
Our discriminator/regressor, defined by a probabilistic
model $p_R(c|x)$ with parameters $\theta_R$ , is a feedforward neural network that learns to map the input feature vector $x \in \mathcal{R}^{D}$ to its
corresponding class-value $c \in \mathcal{R}^{1}$ . The regressor
is learned using two sources of data:
\begin{enumerate}
    \item Labeled examples $\{x_n,c_{y_n}\}^{N}_{n=1}$ from the seen class,
on which we can define a supervised loss, given by
 %
 \begin{equation}
 \mathcal{L}_{Sup}(\theta_R)=-\mathbb{E}_{ \{x_n,c_{y_n} \} }\left[ p_R(c_{y_n}|x_n) \right]
 \end{equation}
 
 
 \item Synthesized examples $\widehat{x}$ from the generator, for which
we can define an unsupervised loss, given by
\begin{equation}
 \mathcal{L}_{Unsup}(\theta_R)=-\mathcal{E}_{p_{\theta_G} (\widehat{x}|z,c)p(z)p(c)} \left[ p_R(c|\widehat{x}) \right]
 \end{equation}
 
 
 Note that the unsupervised loss is computed by tak-
ing a latent code z sampled from the prior p(z), along
with a class-value $c$ sampled from the empirical distribution $p(c)$, generating an exemplar from
the generator distribution $p_{\theta_G}(\widehat{x}|z,c))$, and then taking
an expectation w.r.t. these distributions. During this
phase, we can use attributes both from seen as well as
unseen classes.

The overall training objective of the regressor is then
defined as the following weighted combination of the
supervised and the unsupervised training objectives
%
\begin{equation}
    \min_{\theta_R} \mathcal{L}_R = \mathcal{L}_{Sup} + \lambda_R \cdot \mathcal{L}_{Unsup}
\end{equation}

The above optimization problem is the first step of the
alternating optimization procedure. It optimizes the regressor parameters $\theta_R$ to make the regressor predict
the correct class-value even with a noisy signal $\widehat{x}$. Note that, in this step, we assume that the generator distribution is fixed.

\end{enumerate}




\subsubsection{Generator Network}


The conditional VAE of our architecture con-
sists of the conditional generator $p_G (x|z,c)$ with parameters $\theta_G$  which generates synthetic features to train the classifier 
% Hence the training needs to be designed such
% that the generated class conditional distribution nicely ap-
% proximates the true distribution. 
Denoting the VAE encoder as $p_E(z|x)$ with parameters $\theta_E$ , and the regressor output distribution as $p_R(c|x)$, the VAE loss function is given by
% (assuming the regressor to be fixed)
%
\begin{equation}
\begin{split}
    \mathcal{L}_{VAE}(\theta_E,\theta_G)= -\mathcal{E}_{p_E(z|x),p(c|x)}\left[\log p_G(x|z,c)\right] \\
    + KL(p_E(z|x)||p(z))
\end{split}
\end{equation}
%
where the first term on the R.H.S. is the generator’s reconstruction error and the second term promotes the VAE posterior (the encoder) to be close to the prior. 

We model the VAE encoder $p_E(z|x)$, VAE conditional
decoder/generator $p_G(x|z, c)$, and the regressor $p_R(c|x)$
as Gaussian distributions. The factorization
of the joint distribution over overall latent code $(z, c)$ into
two components $p_E(z|x)$ and $p_R(c|x)$ is consistent with
our attempt at learning a disentangled representation \cite{verma11} to avoid posterior collapse.


\paragraph{Discriminator-Driven Learning:}
%
As described in Sec. 4.1, we use the discriminator/regressor to improve the
generator by backpropagating its error that encourages generation of exemplars, $\widehat{x}$  coherent with the class-value $c$.
We perform this by using a couple of loss functions. The
first one assumes the regressor, has optimal parameters and is defined as:
% any reason for it not regressing to the correct
% value is because of the poor generation by the generator:
%
\begin{equation}
 \mathcal{L}_c(\theta_G)=-\mathcal{E}_{p_G(widehat{x}|z,c)p(z)p(c)}\left[\log p_R(c|\widehat{x}) \right]   
\end{equation}

This loss encourages the generator to create samples such
that the regressed class value by the discriminator is
correct. We also add an additional term that acts as a reg-
ularizer that encourages the generator to generate a good
class-specific sample even from a random z drawn from
the prior p(z) and combined with class-attribute from p(c).
%
\begin{equation}
 \mathcal{L}_{Reg}(\theta_G)=-\mathcal{E}_{p(z)p(c)}\left[\log p_G(\widehat{x}|z,c) \right]   
 \label{eq:lreg}
\end{equation}

The above ensures that the quality of the synthesized features is similar to the actual data. While the above two loss functions help us
increase the coherence of $\widehat{x} ~ p_G (\widehat{x}|z,c)$ with the class-value $c$, we also need to enforce the independence (dis-
entanglement) \cite{verma11} of $z$ from
the class-value $c$. The encoder 
ensures that the sampling distribution and the one obtained
from the generated exemplar follow the same distribution.
More formally, we add a loss component,
%
\begin{equation}
 \mathcal{L}_{E}(\theta_G)=-\mathcal{E}_{\widehat{x} ~ p_G (\widehat{x}|z,c)} KL\left[\log p_E(z|\widehat{x})||q(z) \right]   
 \label{eq:le}
\end{equation}
%
The distribution $q(z)$ could be the prior $p(z)$ or the posterior
from a labeled sample $p(z|x_n)$%, in which case the  class-value ute
% component a y n is used. 
Hence the complete learning objective for the generator and encoder is given by,
%
\begin{equation}
    \min_{\theta_G,\theta_E} \mathcal{L}_{VAE} + \lambda_c \cdot \mathcal{L}_c + \lambda_{reg} \cdot \mathcal{L}_{reg} + \lambda_E \cdot \mathcal{L}_E
\end{equation}

The overall learning objective for the conditional auto-
encoder is a weighted combination of all the components
discussed above, effectively optimizing parameters to en-
sure good density estimation. Vanilla conditional genera-
tive models like conditional VAE [21] and [3] crucially lack
such a mechanism. The weight are hyperparameters, tuned
for optimal reconstruction.



%  A common choice for generative models is to use  Generative Adversarial
% Nets (GANs) \cite{GANs}. However, as reported in \cite{Huang30}, conditional variational auto encoders (CVAE) can better map noise vectors to image features.
% In our proposed framework the CVAE consists
% of two parts, an encoder $P_E(F^{output}|F^{input},r^{input})$ that maps the base feature vector $F^{input}$ of known class value $r^{input}$, to an output feature vector $F^{output}$. The second component of the CVAE is the decoder/generator $P_G(F^{input}|F^{output}, c)$ that maps the output vector (or the synthesized feature vector) to a class value 
% data point. The training objective of CVAE is to minimize
% the following loss function:
% \begin{equation}
%     CVAE
% \end{equation}
% where DKL(p||q) represents the Kullback-Leibler divergence
% between two distributions p and q, and P(z) is treated
% as a unit Gaussian distribution.


% However, as pointed out in [41, 40, 8, 21], CVAE is hard
% to train due to the posterior collapse problem. In order to
% mitigate this problem, we follow [31] to disentangle z from
% c, so that the encoder only depends on x (i.e. PG(z|x)), as
% illustrated in the top left of Figure 3. Also, as in [21], we
% add an adversarial loss to help learning better CVAE, which
% we will discuss later. The loss of the conditional variational
% autoencoder (CVAE) used in our model is defined as follows:
% LCVAE(E, G) = E
% Pdata(v,s),PE(z|v)[log PG(v|z, s)] (2)
% − DKL(PE(z|v)||P(z)),

% where v is an image’s visual feature and s is the class embedding
% of v.
% Although generative models like VAE [16] and
% GAN [12] have been proved to be effective in generating
% images, the output images of generative models are still
% blurry for images with complex objects, and the synthetic
% images often lack the sharpness to reveal the detailed attributes
% of objects, which are important for zero-shot learning
% [7]. Hence, instead of generating raw images, we train
% CVAE to generate visual feature v, where the ground truth
% visual features are provided by image classification models
% pretrained on ImageNet [28].



\subsection{Training and Implementation}

The network was optimized based
on the loss function discussed in Sec. 4, using the Adam
[13] optimizer. The learning started with pre-training the
VAE using the loss from Eq. 4. This is followed by joint
alternating-training of regressor and encoder-generator pair
by optimizing the loss from Eq. 3 and Eq. 8, until conver-
gence. The hyerparameters were chosen based on a train-
validation split and were used while training the model on
complete data. Though there may be some small variabil-
ity in the results based on the values for the hyperparam-
eters, we used $\lambda_R$ = 0.1, $\lambda_c$ = 0.1, $\lambda_{reg}$ = 0.1 and
$\lambda_E$ = 0.1, which worked well for most of the experiments.
It is important to note that the same architecture is used
across all datasets and no extra data/feature engineering is
used/performed to improve accuracies, thus showcasing the
efficacy of the training schedule for this task. The encoder
is realised using a two-hidden layer feedforward network
while the decoder and the regressor are modeled as feed-
forward networks consisting of one hidden layer with 512
hidden units each.
For the evaluation criteria, we use the average per-class
accuracy. This metric reduces the bias of classes having
higher examples in the test set, and provides a better mea-
sure of the model performance [34].
We shall now discuss the experimental setup for the
two settings we experiment with: ZSL and GZSL. Let the
datasets be available in two parts, the labeled examples from
the seen classes, X S and the unlabeled examples from the
unseen classes, X U .



\subsection{ Evaluation Protocol}

Once the model has been trained, in order to predict the
label for unseen classes, we can first generate new samples
for each unseen class, and then combine those synthetic
samples with other samples in the training data, after which
we can train any new classifier based on this new dataset
that contains samples for both seen and unseen classes. 


3.4 Learning and Testing
As shown in [1] the training of a classifier using a potentially unlimited num-
ber of samples from the seen and unseen classes generated with x ~ G(a, z; $\theta_G$
)
produces more accurate classification results compared with multi-modal em-
bedding models [18–21]. Therefore, we train a final softmax classifier P(y|x, $\theta_C$),
defined in (4), using the generated visual features by minimizing the negative log
likelihood loss $\ell_{CLS}$( $\theta_C, \theta_G$
), as defined in (3), where $\theta_G$
has been learned from
one of the feature learning strategies discussed in Sec. 3.3 - the training of the
classifier produces $\theta_c$
. The samples used for training the classifier are generated
based on the task to be solved. For instance, for ZSL, we only use generated
visual representations from the set of unseen classes; while for GZSL, we use the
generated samples from seen and unseen classes.
Finally, the testing is based on the prediction of a class for an input test
visual representation x, as follows:
y = arg max
y2 e Y
P(y|x, $\theta$.C
), (9)
where e Y = Y for GZSL or e Y = YU for ZSL.



==> misc.tex <==
\subsection{Problem Formulation}

In the GZSL+DG problem, the goal is to recognize unseen categories (as in GZSL)
in unseen domains (as in DG). Formally, let $\mathcal{X}$ denote the input image space, $\mathcal{Y}$ denote the set of possible classes and $\mathcal{D}$ the set of possible domains.
At training time, we have $\mathcal{S} = \{(x_i, y_i, d_i )\}^{n}_{i=1}$ where $x_i \in \mathcal{X}, y_i \in \mathcal{Y}^{s}$, and $d_i \in \mathcal{D}^{s}$. Here the superscript $s$ denotes the seen classes and $\mathcal{Y}^{s}\subset \mathcal{Y}, \mathcal{D}{s} \subset \mathcal{D}$. There can be multiple source domains with different 
distributions $p_{\mathcal{X}}(x|d_i) \neq p_{\mathcal{X}}(x|d_j)$, $\forall i \neq j$.


Given $\mathcal{S}$ we aim to mapping $h$ from image $x \in \mathcal{D}^{u}$  to its corresponding label from $\mathcal{Y}^{u} \subset \mathcal{Y}$. In the case of GZSL the domains as  well as labels are shared across the test and training datasets. The set of labels observed during training can be denoted as $\mathcal{Y}^{s}$ (the seen label set) while the set of labels observed at test time is $\mathcal{Y}^{s} \cup \mathcal{Y}^{u}$, a combination of seen and unseen label set. 


we divide the function h into three parts: f , mapping images
into a feature space Z, i.e. f : X → Z, g going from Z to a semantic embedding
space E, i.e. g : Z → E, and an embedding function ω : Y t → E where Y t ≡ Y s
during training and Y t ≡ Y u at test time. Note that ω is a learned classifier for
DG while it is a fixed semantic embedding function in ZSL, mapping classes into
their vectorized representation extracted from external sources. Given an image
x, the final class prediction is obtained as follows:  

y ∗ = argmax y ω(y) g(f (x)).
(1)
In this formulation, f can be any learnable feature extractor (e.g. a deep neural
network), while g any ZSL predictor (e.g. a semantic projection layer, as in [46]
or a compatibility function among visual features and labels, as in [1,2]). The
first solution to address the ZSL+DG problem could be training a classifier using
the aggregation of data from all source domains. In particular, for each sample
we could minimize a loss function of the form:
X
L AGG (x i , y i ) =
`(ω(y) | g(f (x i )), y i )
(2)
y∈Y s
with ` an arbitrary loss function, e.g. the cross-entropy loss. In the following,
we show how we can use the input to Eq. (2) to effectively recognize unseen
categories in unseen domains.


everse task of mapping visual features
back to their corresponding semantic features. The CVAE
and Regressor together form a dual learning framework so
that they can learn from each other. In our case, the prime
task is generating image features conditioned on class em-
bedding, while the dual task is to transform image features
back to their corresponding class embedding.
As illustrated in the down left of Figure 3, the Regres-
sor network R takes two kinds of image features as input,
where the first kind is the real image features v sampled
from training data, and the second kind is the fake features
v ′ = G(s, z) generated by the CVAE. With the paired train-
ing data (v, s), we can train the Regressor with a supervised
loss:

L sup (R) = E P data (v,s) ||s − R(v)|| 22 .
(3)
In addition, the Regressor interacts with the CVAE with
the following cyclic-consistency loss:
L cyc (θ G , θ E , θ R ) = E P data (v,s),P E (z|v) [||v − G(R(v), z)|| 22
(4)
+ ||s − R(G(s, z))|| 22 ],
where G is the decoder/generator of CVAE and P E (z|v) is
implemented by the encoder E in Figure 3.




---------------------------- NEW Text

==> misc2.tex <==
\section{Method}
\label{sec:method}

Figure~\ref{fig:workflow} depicts the different stages of our proposed approach for combining domain generalization and generalized zero shot learning. 

In this section, we first formalize the Generalized Zero-Shot Learning under Domain Generalization (ZSL+DG). We then describe our approach, $----$ , which, by performing curriculum learning through mixup, simulates the domain- and semantic-shift
the network will encounter at test time. %, and can be holistically applied to ZSL, DG and ZSL+DG.

\subsection{Problem Formulation}

In the GZSL+DG problem, the goal is to recognize unseen categories (as in GZSL)
in unseen domains (as in DG). Formally, let $\mathcal{X}$ denote the input image space, $\mathcal{Y}$ denote the set of possible classes and $\mathcal{D}$ the set of possible domains.
At training time, we have $\mathcal{S} = \{(x_i, y_i, d_i )\}^{n}_{i=1}$ where $x_i \in \mathcal{X}, y_i \in \mathcal{Y}^{s}$, and $d_i \in \mathcal{D}^{s}$. Here the superscript $s$ denotes the seen classes and $\mathcal{Y}^{s}\subset \mathcal{Y}, \mathcal{D}{s} \subset \mathcal{D}$. There can be multiple source domains with different 
distributions $p_{\mathcal{X}}(x|d_i) \neq p_{\mathcal{X}}(x|d_j)$, $\forall i \neq j$.


Given $\mathcal{S}$ we aim to mapping $h$ from image $x \in \mathcal{D}^{u}$  to its corresponding label from $\mathcal{Y}^{u} \subset \mathcal{Y}$. In the case of GZSL the domains as  well as labels are shared across the test and training datasets. The set of labels observed during training can be denoted as $\mathcal{Y}^{s}$ (the seen label set) while the set of labels observed at test time is $\mathcal{Y}^{s} \cup \mathcal{Y}^{u}$, a combination of seen and unseen label set. 


we divide the function h into three parts: f , mapping images
into a feature space Z, i.e. f : X → Z, g going from Z to a semantic embedding
space E, i.e. g : Z → E, and an embedding function ω : Y t → E where Y t ≡ Y s
during training and Y t ≡ Y u at test time. Note that ω is a learned classifier for
DG while it is a fixed semantic embedding function in ZSL, mapping classes into
their vectorized representation extracted from external sources. Given an image
x, the final class prediction is obtained as follows:  

y ∗ = argmax y ω(y) g(f (x)).
(1)
In this formulation, f can be any learnable feature extractor (e.g. a deep neural
network), while g any ZSL predictor (e.g. a semantic projection layer, as in [46]
or a compatibility function among visual features and labels, as in [1,2]). The
first solution to address the ZSL+DG problem could be training a classifier using
the aggregation of data from all source domains. In particular, for each sample
we could minimize a loss function of the form:
X
L AGG (x i , y i ) =
`(ω(y) | g(f (x i )), y i )
(2)
y∈Y s
with ` an arbitrary loss function, e.g. the cross-entropy loss. In the following,
we show how we can use the input to Eq. (2) to effectively recognize unseen
categories in unseen domains.


---------------------------- NEW Text

\subsection{Method Overview}

Let us consider the scenario where we have available histopathology images of PCa with know gleason grades of $1,2,3$. We are interested to develop a method that can recognize, from the test set, samples of gleason grades $4,5$ in addition to grades $1,2,3$. The above is a case of generalized zero shot learning.  This is a realistic scenario since it is challenging to obtain sufficiently labeled samples for a wide variety of disease cases. Although in this example we have taken grades $1,2,3$ as available samples, in reality the available grades can be one or more from the grading scale. 




Existing ZSL models only see labeled data from seen
classes during training biasing the predictions to seen
classes. The main insight of our proposed model is that
by feeding additional synthetic CNN features of unseen
classes, the learned classifier will also explore the embed-
ding space of unseen classes. Hence, the key to our ap-
proach is the ability to generate semantically rich CNN fea-
ture distributions conditioned on a class specific semantic
vector e.g. attributes, without access to any images of that
class. This alleviates the imbalance between seen and un-
seen classes, as there is no limit to the number of synthetic
CNN features that our model can generate. It also allows to
directly train a discriminative classifier, i.e. Softmax classi-
fier, even for unseen classes.

We begin by defining the problem of our interest. Let
S = {(x, y, c(y))|x ∈ X , y ∈ Y s , c(y) ∈ C} where
S stands for the training data of seen classes, x ∈ R d x
is the CNN features, y denotes the class label in Y s =
{y 1 , . . . , y K } consisting of K discrete seen classes, and
c(y) ∈ R d c is the class embedding, e.g. attributes, of class
y that models the semantic relationship between classes.
In addition, we have a disjoint class label set Y u =
{u 1 , . . . , u L } of unseen classes, whose class embedding set
U = {(u, c(u))|u ∈ Y u , c(u) ∈ C} is available but images
and image features are missing. Given S and U , the task of
ZSL is to learn a classifier f zsl : X → Y u and in GZSL we
learn a classifier f gzsl : X → Y s ∪ Y u .

3.1. Feature Generation
In this section, we begin our discussion with Generative
Adversarial Networks (GAN) [18] for it being the basis of
our model. GAN consists of a generative network G and
a discriminative network D that compete in a two player
minimax game. In the context of generating image pixels,
D tries to accurately distinguish real images from generated
images, while G tries to fool the discriminator by generat-
ing images that are mistakable for real. Following [29], we
extend GAN to conditional GAN by including a conditional
variable to both G and D. In the following we give the de-
tails of the conditional GAN variants that we develop. Our
novelty lies in that we develop three conditional GAN vari-
ants, i.e. f-GAN, f-WGAN and f-CLSWGAN, to generate
image features rather than image pixels. It is worth noting
that our models are only trained with seen class data S but
can also generate image features of unseen classes.


f-GAN. Given the train data S of seen classes, we aim to
learn a conditional generator G : Z × C → X , which takes
random Gaussian noise z ∈ Z ⊂ R d z and class embedding
c(y) ∈ C as its inputs, and outputs a CNN image feature x̃ ∈
X of class y. Once the generator G learns to generate CNN
features of real images, i.e. x, conditioned on the seen class
embedding c(y) ∈ Y s , it can also generate x̃ of any unseen
class u via its class embedding c(u). Our feature generator
f-GAN is learned by optimizing the following objective,
min max L GAN =E[log D(x, c(y))]+
G
discriminator
CNN
z ~ N(0, 1)
f-CLSWGAN
generator
Head color: brown
Belly color: yellow
Bill shape: pointy
Figure 2: Our f-CLSWGAN: we propose to minimize
the classification loss over the generated features and the
Wasserstein distance with gradient penalty.
between pairs of real and generated points. Again, we solve
a minmax optimization problem,
min max L W GAN
G
D
(3)
f-CLSWGAN. f-WGAN does not guarantee that the gener-
ated CNN features are well suited for training a discrimi-
native classifier, which is our goal. We conjecture that this
issue could be alleviated by encouraging the generator to
construct features that can be correctly classified by a dis-
criminative classifier trained on the input data. To this end,
we propose to minimize the classification loss over the gen-
erated features in our novel f-CLSWGAN formulation. We
use the negative log likelihood,
(1)
D
L CLS = −E x̃∼p x̃ [log P (y|x̃; θ)],
E[log (1 − D(x̃, c(y)))],
with x̃ = G(z, c(y)). The discriminator D : X × C →
[0, 1] is a multi-layer perceptron with a sigmoid function
as the last layer. While D tries to maximize the loss, G
tries to minimizes it. Although GAN has been shown to
capture complex data distributions, e.g. pixel images, they
are notoriously difficult to train [4].


f-WGAN. We extend the improved WGAN [19] to a con-
ditional WGAN by integrating the class embedding c(y) to
both the generator and the discriminator. The loss is,
L W GAN =E[D(x, c(y))] − E[D(x̃, c(y))]−
(2)
2
λE[(||∇ x̂ D(x̂, c(y))|| 2 − 1) ],
where x̃ = G(z, c(y)), x̂ = αx + (1 − α)x̃ with α ∼
U (0, 1), and λ is the penalty coefficient. In contrast to the
GAN, the discriminative network here is defined as D : X ×
C → R, which eliminates the sigmoid layer and outputs a
real value. The log in Equation 1 is also removed since we
are not optimizing the log likelihood. Instead, the first two
terms in Equation 2 approximate the Wasserstein distance,
and the third term is the gradient penalty which enforces
the gradient of D to have unit norm along the straight line


between pairs of real and generated points. Again, we solve
a minmax optimization problem,
min max L W GAN
G
D
(3)
f-CLSWGAN. f-WGAN does not guarantee that the gener-
ated CNN features are well suited for training a discrimi-
native classifier, which is our goal. We conjecture that this
issue could be alleviated by encouraging the generator to
construct features that can be correctly classified by a dis-
criminative classifier trained on the input data. To this end,
we propose to minimize the classification loss over the gen-
erated features in our novel f-CLSWGAN formulation. We
use the negative log likelihood,

where x̃ = G(z, c(y)), y is the class label of x̃, P (y|x̃; θ)
denotes the probability of x̃ being predicted with its true
class label y. The conditional probability is computed by a
linear softmax classifier parameterized by θ, which is pre-
trained on the real features of seen classes. The classifica-
tion loss can be thought of as a regularizer enforcing the
generator to construct discriminative features. Our full ob-
jective then becomes,
min max L W GAN + βL CLS
G
D
(5)
where β is a hyperparameter weighting the classifier.


3.2. Classification
Given c(u) of any unseen class u ∈ Y u , by resampling
the noise z and then recomputing x̃ = G(z, c(u)), arbitrar-
ily many visual CNN features x̃ can be synthesized. After
repeating this feature generation process for every unseen
class, we obtain a synthetic training set Ũ = {(x̃, u, c(u))}.
We then learn a classifier by training either a multimodal
embedding model or a softmax classifier. Our generated
features allow to train those methods on the combinations
of real seen class data S and generated unseen class data Ũ .

Multimodal Embedding. Many zero-shot learning
approaches, e.g. ALE [2], DEVISE [14], SJE [3], ES-
ZSL [40] and LATEM [45], learn a multimodal embedding
between the image feature space X and the class embedding
space C using seen classes data S. With our generated fea-
tures, those methods can be trained with seen classes data S
together with unseen classes data Ũ to learn a more robust
classifier. The embedding model F (x, c(y); W ), parameter-
ized by W , measures the compatibility score between any
image feature x and class embedding c(y) pair. Given a
query image feature x, the classifier searches for the class
embedding with the highest compatibility via:
f (x) = argmax F (x, c(y); W ),
(6)
y
where in ZSL, y ∈ Y u and in GZSL, y ∈ Y s ∪ Y u .
Softmax. The standard softmax classifier minimizes the
negative log likelihood loss,
min −
θ
1
|T |
X
log P (y|x; θ),
(7)
(x,y)∈T
where θ ∈ R d x ×N is the weight matrix of a fully con-
nected layer which maps the image feature x to N unnor-
malized probabilities with N being the number of classes,
and P (y|x; θ) =
exp(θ y T x)
P N
.
T
i exp(θ i x)
Depending on the task,
T = Ũ if it is ZSL and T = S ∪ Ũ if it is GZSL. The
prediction function is:
f (x) = arg max P (y|x; θ),
y
(8)
where in ZSL, y ∈ Y u and in GZSL, y ∈ Y s ∪ Y u






==> misc3.tex <==
\section{Method}
\label{sec:method}

Figure~\ref{fig:workflow} depicts the different stages of our proposed approach for combining domain generalization and generalized zero shot learning. 

In this section, we first formalize the Generalized Zero-Shot Learning under Domain Generalization (ZSL+DG). We then describe our approach, $----$ , which, by performing curriculum learning through mixup, simulates the domain- and semantic-shift
the network will encounter at test time. %, and can be holistically applied to ZSL, DG and ZSL+DG.

\subsection{Problem Formulation}

In the GZSL+DG problem, the goal is to recognize unseen categories (as in GZSL)
in unseen domains (as in DG). Formally, let $\mathcal{X}$ denote the input image space, $\mathcal{Y}$ denote the set of possible classes and $\mathcal{D}$ the set of possible domains.
At training time, we have $\mathcal{S} = \{(x_i, y_i, d_i )\}^{n}_{i=1}$ where $x_i \in \mathcal{X}, y_i \in \mathcal{Y}^{s}$, and $d_i \in \mathcal{D}^{s}$. Here the superscript $s$ denotes the seen classes and $\mathcal{Y}^{s}\subset \mathcal{Y}, \mathcal{D}{s} \subset \mathcal{D}$. There can be multiple source domains with different 
distributions $p_{\mathcal{X}}(x|d_i) \neq p_{\mathcal{X}}(x|d_j)$, $\forall i \neq j$.


Given $\mathcal{S}$ we aim to mapping $h$ from image $x \in \mathcal{D}^{u}$  to its corresponding label from $\mathcal{Y}^{u} \subset \mathcal{Y}$. In the case of GZSL the domains as  well as labels are shared across the test and training datasets. The set of labels observed during training can be denoted as $\mathcal{Y}^{s}$ (the seen label set) while the set of labels observed at test time is $\mathcal{Y}^{s} \cup \mathcal{Y}^{u}$, a combination of seen and unseen label set. 


we divide the function h into three parts: f , mapping images
into a feature space Z, i.e. f : X → Z, g going from Z to a semantic embedding
space E, i.e. g : Z → E, and an embedding function ω : Y t → E where Y t ≡ Y s
during training and Y t ≡ Y u at test time. Note that ω is a learned classifier for
DG while it is a fixed semantic embedding function in ZSL, mapping classes into
their vectorized representation extracted from external sources. Given an image
x, the final class prediction is obtained as follows:  

y ∗ = argmax y ω(y) g(f (x)).
(1)
In this formulation, f can be any learnable feature extractor (e.g. a deep neural
network), while g any ZSL predictor (e.g. a semantic projection layer, as in [46]
or a compatibility function among visual features and labels, as in [1,2]). The
first solution to address the ZSL+DG problem could be training a classifier using
the aggregation of data from all source domains. In particular, for each sample
we could minimize a loss function of the form:
X
L AGG (x i , y i ) =
`(ω(y) | g(f (x i )), y i )
(2)
y∈Y s
with ` an arbitrary loss function, e.g. the cross-entropy loss. In the following,
we show how we can use the input to Eq. (2) to effectively recognize unseen
categories in unseen domains.




\subsection{Method Overview}

Let us consider the scenario where we have available histopathology images of PCa with know gleason grades of $1,2,3$. We are interested to develop a method that can recognize, from the test set, samples of gleason grades $4,5$ in addition to grades $1,2,3$. The above is a case of generalized zero shot learning.  This is a realistic scenario since it is challenging to obtain sufficiently labeled samples for a wide variety of disease cases. Although in this example we have taken grades $1,2,3$ as available samples, in reality the available grades can be one or more from the grading scale. 


We have available magnetic resonance imaging (MRI) data of the same patient corresponding to the histopathology images of grades $1,2,3$. MRI images being non-invasive are easier to acquire than histopathology images. On the other hand MRI can be acquired at an early stage of disease while histopathology images are obtained only after tissue resection at an much advanced stage of disease. However, histopathology images are considered the best and most accurate modality for PCa staging. On the other hand MRI images may sometimes miss certain disease signatures due to their inherent low resolution and device noise. 

This presents us with contradictory settings- while MRI is easy to acquire it does not provide very accurate staging; although histopathology images will provide accurate diagnosis they are not easily obtained. Hence it would be beneficial if the MRI images could be supplemented with features from the histopathology images

This is also a case of domain generalization where the training set has data from one domain (MRI images of grades $1,2,3$) while the test set has images from grades $4,5$ in addition to grades $1,2,3$. Additionally, we aim to integrate features from histopathology images since they provide a rich source of information for disease diagnosis. 
Thus we propose a novel approach for combining GD and GZSL for PCa detection. Our approach has the following steps:
\begin{enumerate}
    \item Take MRI of grades 1,2,3
    \item generate MRI features and the corresponding histopahtology features
    \item use histopathology features to generate histopathology images
    \item generate unseen class MRI and unseen class DP by feature extrapolation/mixing
    \item use both images for training a classification system
\end{enumerate}


\subsection{Generating common representations for RI and DP}

\subsection{novel method for synthetic image generation for GZSL using self supervised learning/OCD}

\subsection{Generating novel images}



==> misc4.tex <==
\section{Method}
\label{sec:method}



% \subsection{Method Overview}
\subsection{ Method Overview}

Figure~\ref{fig:workflow} depicts our proposed workflow. Given a set of histopathology images,$I^{DP}$, with known Gleason grades and the corresponding set of MR images $I^{MRI}$ from the same patients, our objective is to learn a method to leverage DP and MR image features for predicting Gleason grades of a test image which may come from seen and unseen classes.

 

$I^{DP}$ and $I^{MRI}$ are both passed through a feature generator to obtain feature vectors, denoted as $F^{DP}$ and $F^{MRI}$, which has two uses. The first use is to train a cycleGAN which learns to generate $F^{DP}$ from $F^{MRI}$ and vice-versa. % set of features from the other.
%
The second use of the feature vectors $F^{DP}$ and $F^{MRI}$ is to train a regressor to predict the class label as a real value. The regressor also acts as a discriminator providing feedback to the feature generator such that the generated features are optimal for the task of predicting Gleason grades.


\textbf{revisit later}

We have a separate feature synthesizer network which takes as input a base feature vector alongwith its class value, and the desired class vallue of the output feature vector. Here, we refer to the Gleason grade as class value since we map the grades to the real value space. The generator part generates a feature vector while a regressor acts as a discriminator providing feedback on the output and helping to train the generator. Using this feature synthesizer we generate samples of the seen and unseen classes which are used to train a classifier for predicting label of test images. 


\begin{figure}[t]
 \centering
\begin{tabular}{cc}
\includegraphics[height=4cm, width=8.5cm]{Figures/Workflow1.png}  \\
(a)\\
\end{tabular}
\caption{Workflow diagram of proposed method.}
\label{fig:workflow}
\end{figure}



% The work by Huang et al. \cite{HuangDualGAN} describes a Generative Dual
% Adversarial Network (GDAN) which can be considered the state of the art in generative methods for GZSL.  They use three components - a Generator, a
% Regressor and a Discriminator. The core component 
% is the Generator network that can generate various
% visual features conditioned on class labels. 
% The Regressor network acts
% as a deep embedding function, which maps each visual
% feature back to the corresponding class’s semantic feature or attribute vector.
% %
% The Generator and the Regressor network together
% form a dual learning framework, so that they can learn
% from each other through a cyclic consistency loss. 
% The Discriminator network that measures
% the similarity of a visual-textual feature pair, and it
% interacts with the other two networks through a dual adversarial loss. 





% Due to the fact that it is very challenging to obtain meaningful attribute vectors for medical images, we propose a novel architecture that leverages domain knowledge.

 

% Figure~\ref{fig:workflow} shows the different steps of our proposed method. The image is input to a GAN module which generates features that act as input to the ordinal regressor which learns to predict the different severity values. We train this part of the network comprising GAN and regressor together in an end to end manner since we wish to learn features that are optimal for ordinal regression, and pre-trained networks do not provide such optimal feature vectors. 

We also have a discrminator network to determine whether it is the right label or not.




\subsection{Problem Definition and Notations}

We consider the scenario with available histopathology and MR images of PCa with known Gleason grades of $1,2,3$, and aim to train a network that can correctly classify from the test set (consisting of MR images) samples of Gleason grades $4,5$ in addition to grades $1,2,3$. The above is a case of generalized zero shot learning and is a realistic scenario since: 1) it is challenging to obtain sufficiently labeled histopathology images for a wide variety of disease cases; 2) MRI, being non-interventional,  is easily obtained compared to histopathology images; 3) it is beneficial to make decisions based on the combination of histopathology and MRI since histopathology images provide better information due to their high resolution. Although in this example we have taken grades $1,2,3$ as available classes, in reality the available grades can be one or more from the Gleason scale.


Let us denote the training data  as $S = {(\textbf{v}, y, \textbf{s}_y)}$ , where $v \in \mathcal{V}^{s}$ is the image feature  and $\mathcal{V}^{s}$ is the set of image features from the seen classes; $y\in \mathcal{Y}^{s}$ is the label of $\textbf{v}$ and $\mathcal{Y}^{s}$ is the set of labels for seen classes; $\textbf{s}_y \in \mathcal{A}$ is the attribute vector  (semantic embedding) for class $y$.  Similarly, we can define the test
set as $U = {(\textbf{v}, y, \textbf{s}_y)}$, where $v \in \mathcal{V}^{u}$  and $\mathcal{V}^{u}$ is the set of image features from the unseen classes; $y\in \mathcal{Y}^{u}$, $\mathcal{Y}^{u}$ is the set of labels for unseen classes and $\mathcal{Y}^{s} \cap \mathcal{Y}^{u}=\emptyset$. In GZSL we aim to learn a classifier that maps an image feature vector $\textbf{v}$ to a seen or unseen class, i.e., $f:\textbf{v} \xrightarrow[]{} \mathcal{Y}^{s} \cup \mathcal{Y}^{u}$.

Below we describe different components of our proposed network.

\subsection{Feature Extractor Network/Feature Generation Network}


An important component of GZSL methods is the availability of a class attribute vector that defines the characteristics of the seen and unseen classes. However in medical images it is extremely challenging to obtain a descriptive attribute vector due to time constraints of clinical experts. Moreover it is not trivial to describe any class (seen or unseen) by class attribute vectors since the same class may have different attribute vectors. Our method's novelty is it can perform GZSL without the need for class attribute vectors.


The first step is to extract features from the histopathology and MR images. We choose to work on image features instead of original images because: 1) in the case of the output images of generative models are still
blurry for images with complex objects, and the synthetic
images often lack the sharpness to reveal the detailed attributes
of objects, which are important for zero-shot learning
\cite{huang7}. Hence, instead of generating raw images, we train
CVAE to generate visual feature v,

2) generating high resolution histopathology images from low resolution and noisy MRI is an extremely challenging task and it is much easier to find a correlation between their feature vectors.

We use a pre-trained network with the VGG architecture that has been pre-trained on the CAMELYON17 dataset.

We also consider an alternative approach by training an end to end network. (ablation studies)






A common choice for generative models is to use  Generative Adversarial
Nets (GANs) \cite{GANs}. However, as reported in \cite{HUang30}, conditional variational auto encoders (CVAE) has a better ability to map noise vectors to  image features.
A CVAE consists
of two parts, an encoder $P_E(z|x,c)$ that maps a data point x, along with its class feature c, to its latent feature z, and a
decoder/generator PG(x|z, c) that maps a latent vector to a
data point. The training objective of CVAE is to minimize
the following loss function:
\begin{equation}
    CVAE
\end{equation}
where DKL(p||q) represents the Kullback-Leibler divergence
between two distributions p and q, and P(z) is treated
as a unit Gaussian distribution.


However, as pointed out in [41, 40, 8, 21], CVAE is hard
to train due to the posterior collapse problem. In order to
mitigate this problem, we follow [31] to disentangle z from
c, so that the encoder only depends on x (i.e. PG(z|x)), as
illustrated in the top left of Figure 3. Also, as in [21], we
add an adversarial loss to help learning better CVAE, which
we will discuss later. The loss of the conditional variational
autoencoder (CVAE) used in our model is defined as follows:
LCVAE(E, G) = E
Pdata(v,s),PE(z|v)[log PG(v|z, s)] (2)
− DKL(PE(z|v)||P(z)),

where v is an image’s visual feature and s is the class embedding
of v.
Although generative models like VAE [16] and
GAN [12] have been proved to be effective in generating
images, the output images of generative models are still
blurry for images with complex objects, and the synthetic
images often lack the sharpness to reveal the detailed attributes
of objects, which are important for zero-shot learning
[7]. Hence, instead of generating raw images, we train
CVAE to generate visual feature v, where the ground truth
visual features are provided by image classification models
pretrained on ImageNet [28].


Figure~\ref{fig:workflow} shows the architecture of the CVAE which consists of an encoder and decoder. The encoder consists of 3 convolution blocks with each block consisting of $2$ convolution layers followed by batch normalization and a max pooling layer. The output from the final convolution block is connected to $2$ successive fully connected layers which outputs a $256$ dimensional latent vector which acts as an input to the decoder stage which has symmetrical fully connected layers followed by convolution blocks to reconstruct the original image/feature vector. The latent vector is the image's visual feature which acts as the input to the ordinal regressor.

Explain the design choice:
Initial few conv blocks are to learn a downscaled representation of the input image.. but we do not reconstruct the image since ..............


\subsection{Feature Transformation Network}

We use cyclic GANs for transforming features of one domain to the other domain. 

Cycle GANs transform an image from domain $ A $ to $B$, and the reverse translation from $ B $ to $ A $ should generate the original input image. 
%
In forward cycle consistency, an image from domain $A$ is translated to domain $B$  by generator $G_{AB}$ expressed as $a\hat{b}=G_{AB}(a)$. Image $a\hat{b}$ is translated back to domain $A$ by $G_{BA}$ to get $\hat{a}=G_{BA}(a\hat{b})$.  Similarly, the original and reconstructed images from $B$ should also match.  Thus the overall cycle consistency loss is: % calculated as 
%
\begin{equation}
    L_{cycle} (G_{AB},G_{BA}) = E_{a} \left\|a -G_{BA}(G_{AB}(a))\right\|_1 + \left\|b -G_{AB}(G_{BA}(b))\right\|_1 +L_{Seg},  
    \label{eq:cyc}
\end{equation}
%
% where $L_{Seg}$ is defined as 
\begin{equation}
    L_{Seg} = \overbrace{L_{FeatMap}(a,\hat{a}) + L_{FeatMap}(b,\hat{b})}^{L_{Seg1}} + \overbrace{L_{FeatMap}(a,a\hat{b}) + L_{FeatMap}(b,b\hat{a})}^{L_{Seg2}}
    \label{eq:segL}
\end{equation}
% 
%



%
Discriminator $D_B$ is employed to distinguish between real image $b$
and generated image $a\hat{b}$ where the adversarial loss in forward cycle, $L_{adv}$, is:
%written as
\begin{equation}
    L_{adv} (G_{AB},D_{B},A,B) = E_{b} \log D_B (b) +  E_{a} \log \left[ \left(1-D_B (G_{AB}(a))\right)\right].
\end{equation}
There also exists a corresponding $L_{adv}(G_{BA},D_A,B,A)$ to distinguish between real image $a$ and generated image $b\hat{a}$
%
Thus the final objective function is: %optimized is 
%
\begin{equation}
    L= L_{adv}(G_{AB},D_B,A,B) + L_{adv}(G_{BA},D_A,B,A) + L_{cyc}(G_{AB},G_{BA})
\end{equation}



\subsubsection{Network Architecture}

All the networks ($G_{AB},G_{BA},Seg_{Sem}$) are based on a UNet architecture \cite{Unet} with a ResNet backbone. Each convolution block has $3$ layers of convolution layers (all using the adaptive pixel convolutions and ELU), followed by a $2\times2$ max-pooling step of stride $2$. Skip connections exist between the stages of the contracting and expanding path. $3\times3$ kernels are used with adequate padding to maintain image dimensions. There are four convolution blocks in both paths.


CycleGANs \cite{CyclicGANs} learn mapping functions $G : X \rightarrow Y$ and $F : Y \rightarrow X$,  between image sets $X=I^{Flt}$ and $Y=I^{Ref}$. Adversarial discriminators $D_X$ differentiate  between images $x$ and registered images ${F(y)}$, and $D_Y$ distinguishes between ${y}$ and ${G(x)}$. %Here $X=I^{Flt}$ and $Y=I^{Ref}$. 
$G$ registers $I^{Flt}$ to $I^{Ref}$ while $F$ is trained to register $I^{Ref}$ to $I^{Flt}$. We refer the reader to \cite{CyclicGANs} for implementation details.
%
In addition to the content loss (Eqn~\ref{eq:conLoss}) we have: 1) an adversarial loss; %to match $I^{Trans}$'s distribution to $I^{Flt}$; 
and 2) a cycle consistency loss to ensure transformations $G,F$ do not contradict each other.
%
%

\paragraph{\textbf{Adversarial Loss}:}


The adversarial loss is an important component to ensure that the generated outputs are plausible. In previous applications the adversarial loss was based on the similarity of generated image to training data distribution. Since our generator network has multiple outputs we have additional terms for the adversarial loss. The first term matches the distribution of $I^{Trans}$ to  $I^{Flt}$  %training data image function ensures that $I^{Trans}$ has similar intensity distribution as $I^{Flt}$, %, and similar spatial shape distribution as , 
and is given by:
%
\begin{equation}
L_{cycGAN}(G,D_Y) = E_{y\in p_{data}(y)} \left[\log D_Y(y)\right] + E_{x\in p_{data}(x)} \left[\log \left(1-D_Y(G(x))\right)\right], 
\label{eqn:cyGan1}
\end{equation}
%
We retain notations $X,Y$ for conciseness.
%
%
%%
 There also exists $L_{cycGAN}(F,D_X)$, the corresponding adversarial loss for $F$ and $D_X$ and is given by  %,  = E_{x\in p_{data}(x)} \left[\log D_X(x)\right] +  E_{y\in p_{data}(y)} \left[\log \left(1-D_X(F(y))\right)\right]$.
%
%
\begin{equation}
L_{cycGAN}(F,D_X) = E_{x\in p_{data}(x)} \left[\log D_X(x)\right] + E_{y\in p_{data}(y)} \left[\log \left(1-D_X(F(y))\right)\right].
\label{eqn:cyGan12}
\end{equation}







Cycle consistency loss ensures that for each $x \in X$ the reverse deformation should bring $x$ back to the original image, i.e. $x \rightarrow G(x) \rightarrow F(G(x))\approx x$. 
Similar constraints also apply for mapping $F$ and $y$. This is achieved using, % the following conditional loss:
%
%\
%
\begin{equation}
%\begin{split}
L_{cyc}(G,F)= E_{x} \left\|F(G(x))-x\right\|_1 + E_{y} \left\|G(F(y))-y\right\|_1,
%\end{split}
\label{eqn:cyGan2}
\end{equation}
%
%w
%

Instead of the original images, $I^{Ref}$ and $I^{Flt}$, we use their latent vector representations as input to the generator to obtain $I^{Trans}$. %Although there are two different CAEs for the input image pair, we have a single CycleGAN model 



\subsection{Ordinal Regressor Network}


Our use case is to predict Gleason grades which is a form of disease severity where the different classes indicate different levels of known disease severity. A severity label of $1$ indicates absence of disease while the label $5$ indicates the most severe condition. Thus there is a progressively increasing severity characteristic of the labels which can be modeled as a ordinal regression problem. 

Suppose the seen classes are $1,2,3$ and the unknown classes are $4,5$. We train an ordinal regressor that learns to predict the different class values. During the feature generation step for unseen classes the feature vectors are perturbed such that the corresponding regressor output is closer to the unknown classes. The feature vectors are then used to train the network to predict seen and unseen classes.


We chose to model the severity levels as a regression problem in this stage in order to generate features that are closer to the unseen classes. The regressor allows us to supervise its output and accordingly perturb feature vectors to produce new features that are closer to the unseen classes. A classifier would not be able to generate features with such granularity. Our approach proves to be more robust than traditional approaches of generating novel features by weighted mixing of existing features. 


While the CVAE learns to generate visual features from
semantic features, our model also has a Regressor network
Conventional DL approaches learn a
multi-class classifier by constraining the instances being
mapped to a real line in order.


However, we take a much simpler approach wherein the class labels are the values to be regressed. In order to incorporate tolerance we have a parameter $\epsilon$ that allows a certain margin within which the outputs can be considered as valid, i.e., samples from diseased class $3$ are allowed to regress to values in the range $[3-\epsilon, 3+\epsilon]$. Value of $\epsilon$ controls the degree of robustness. 

Figure\ref{fig:workflow} shows the regressor network architecture. It takes as input the feature vector from the generator and  network

that performs the r


\subsection{Discriminator Network}

So far, the Generator and Regressor already combines
semantic → visual and visual → semantic methods,
but it still lacks the ability to learn from a flexible metric
which can better evaluate the similarity of features. In order
to incorporate metric learning, the third component of our
model is a Discriminator network D (as shown in the right
of Figure 3) that takes as input a visual-semantic feature pair
(v, s) and output a compatibility score indicating the extent
to which v belongs to the class characterized by s. The
Discriminator network learns how to evaluate the closeness


of an image feature to a class, instead of using a predefined
metric like L1/L2 distance or cosine similarity.
In order to train the Discrimiantor to distinguish differ-
ent types of fake data, inspired by Text-to-Image-GAN [26],
we also train the Discriminator with two kinds of fake in-
put, i.e. (G(s, z), s) and (v, s − ), where s − is a randomly
sampled class’s embedding and s 6 = s − . In addition, we
add a novel third type of fake input generated by the Re-
gressor, i.e. (v, R(v)). In this way, not only the CVAE but
also the Regressor can learn from the Discriminator through
adversarial training.
Since GANs are notoriously hard to train, there are
many methods that try to stabilize the training process of
GAN [12, 22, 4, 13]. In our model, we apply LS-GAN [22]
as the training method for adversarial loss for its simplicity
and effectiveness. Thus the adversarial loss for the Discrim-
inator of our model can be defined as:



where the first term is the loss for real samples (v, s), the
second term stands for the scores of features generated by
the Generator, the third term stands for the scores of class
embedding generated by the Regressor, and the last term is
the control loss which trains the Discriminator to discrimi-
nate pairs of real image features and real negative class em-
bedding. The negative sample s − is randomly sampled from
s −
the set of training classes {s −
y |y ∈ Y , s y 6 = s}. Here the
discriminator D tries to push the scores of real samples to
1 and push the scores for generated samples to 0, while the
generator G tries to push the scores of its synthetic samples
to 1.
Also, the adv



\subsection{Full Objective and Training Procedure}

In adversarial training, the discriminator is training separately
from the other two networks, while we train the
CVAE and Regressor using an overall loss defined as:


where λ 1 , λ 2 and λ 3 are hyper-parameters that assign
weight on different parts of the overall loss.
The training procedure of our GDAN model is as fol-
lows: we first pretrain CVAE using Equation 2, and then
train the whole model in an adversarial way using Equa-
tion 5 and Equation 8. The implementation details will be
provided in the experiment section.



\subsection{Feature Perturbation Network}


The other component of our workflow is the feature perturbation module which perturbs the features of known classes to produce feature vectors of the unknown classes. We propose a self-supervised learning approach for the feature perturbation step ..........
after feature perturbation we check the corresponding output of the regressor. If it is the desired class then we add it to training set. Finally we train a classifier to predict the actual labels in the GZSL setting. .



Our major contribution is a feature perturbation network  whose goal is to generate feature vectors of unseen classes from a base feature vector belonging to a seen class sample.

Given a base feature vector of seen class the objectve is to generate feature vectors that will map to a desired class/disease severity range (e.g. between $[4-\epsilon,4+\epsilon]$. In such a scenario the advantages of using a regressor are clear - given an appropriate network/feature the learned function can map the feature vector to the desired output.

The Feature perturbation network (FPN) takes as input a base feature vector of the seen class, the desired label of the output feature, and a noise vector, to generate an output vector of desired label.

During training we have available the feature vectors of the seen classes....


\subsection{ Evaluation Protocol}
Once the model has been trained, in order to predict the
label for unseen classes, we can first generate new samples
for each unseen class, and then combine those synthetic
samples with other samples in the training data, after which
we can train any new classifier based on this new dataset
that contains samples for both seen and unseen classes. For
fair comparison with other baselines, we just apply a simple
1-NN classifier for testing, which is used in most baselines


